BlindMarket: Enabling Verifiable, Confidential, and Traceable IP Core Distribution in Zero-Trust Settings

We present BlindMarket, an end-to-end zero-trust distribution framework for hardware IP cores. BlindMarket allows two parties, the IP user and the IP vendor, to complete an IP trading process with strong guarantees of verifiability and confidentiality before the transaction, and then traceability after. We propose verification heuristics and adapt the cone of influence-based design pruning to overcome the limited scalability common to cryptographic protocols and the hardness of the underlying hardware verification. We systematically evaluate our framework on a diverse set of real-world hardware benchmarks, and the results demonstrate that BlindMarket effectively completes across a diverse set of real-world hardware IP cores, demonstrating successful verification on 12 out of 13 designs and substantial performance improvements enabled by design pruning and control-flow guided heuristics.

==> draft.tex <==
\newpage
\textbf{Motivating Example.}
Microcontroller-based automation systems are rapidly growing in various traditional low-tech fields, including healthcare\cite{nourizadeh2009medical}, home automation\cite{asadullah2016overview}, and agriculture\cite{edan2009automation}. There are various companies that provide tailored services for those who require embedded automation systems.
% For example, in the agriculture industry, farmers need to continually monitor their crops' real-time cultivation and storage conditions. With the help of an automation system, users can stay updated on crop status in real-time, receive automatic alerts, and even access predictive modeling. 
For example, the automation system in the agriculture industry is designed to optimize grain quality, prevent spoilage, and reduce energy costs. This can be only achieved via embedded automation systems that provide customized service. In practice, however, companies specializing in customized personal services usually don't specialize in chip customization. Instead, they prefer to obtain cost-effective third-party chips that meet their design requirements. These chips often come with various interfaces, including serial communication ports, ADC modules, Bluetooth modules, Wi-Fi modules, and more. However, not every interface is helpful for particular hardware components. An instance of this is that the units used for data collection do not need to have wireless communication capabilities, while those used for data processing do not rely on external sensors. Therefore, during the pre-silicon stage, verification engineers can focus on validating only the necessary functionality of the IP. 

% via multi-level embedded hardware, such as microcontrollers, sensors, and communication networks, which work together that are specialized for a particular service. 
% To achieve this, the system utilizes multi-level embedded hardware, such as microcontrollers, sensors, and communication networks, which work together to collect, transmit, compute, and analyze data.

companies specializing in customized personal services usually don't specialize in chip customization. Instead, they prefer to obtain cost-effective third-party chips that meet their design requirements. These chips often come with miscellaneous interfaces, including serial communication ports, ADC modules, Bluetooth modules, Wi-Fi modules, and more. However, not every interface is useful for particular hardware components. An instance of this is that the units used for data collection do not need to have wireless communication capabilities, while those used for data processing do not rely on external sensors. Therefore, during the pre-silicon stage, verification engineers can focus on validating only the necessary functionality of the IP. This approach saves time and resources.

Assuming that the IP vendor possesses the RTL design, as displayed in Listing \ref{lst:verilogtop}. This submodule is a microcontroller similar to the ESP32 \cite{esp32refmanual}. It offers various APIs, such as I2C, Bluetooth, UART, SPI, ADC, and more. The controller's functionality can be enabled based on the input signal \lstinline[style=vcode]{control}. The output register \lstinline[style=vcode]{state} provides four simplified functionalities: Debug, Bluetooth, I2C, and UART.

\ning{too much irrelavent information}
Traditionally, the Algritech company, as the IP user who needs to purchase the IP design from the IP vendor, chooses to use a wired protocol to build a centralized network for smart agriculture. To collect humidity and temperature data, the user used to utilize an I2C port to link the SHT35\cite{Sensirion_Humidity_Sensors} sensor and a UART port to transmit the collected data to the upstream MKE18F\cite{KE1xFP100M168SF0} for data aggregation. The assertions designed for I2C and UART are checked by the user for practical use. However, this tree-based network suffers from a single point of failure and limited scalability, Algritech decides to upgrade its upcoming system by replacing the current centralized network with a wireless Bluetooth-based mesh network\cite{cilfone2019wireless}. The UART port, which was previously utilized for data transmission, is now being substituted by the Bluetooth module. Thus, the functional assertion \lstinline[style=vcode]{assert property (control == 4'b0001 |-> state == 2'b01)} is now being used for Bluetooth verification.

In this scenario, the bidirectional privacy protocol plays an important role. The IP vendor wants to prevent the hardcoded password 4'b1111 from being exposed, as it could potentially be used as an unauthorized access point to the chip. Additionally, they are concerned about the risks associated with IP theft and piracy. In order to ensure the security and protection of their intellectual property, they prefer to release the design code only after the completion of the business contract, taking necessary precautions.

Previously, IP users relied on I2C and UART functionalities for tree-based networks. However, their future system evolved into a mesh-based network. If the IP user shares their modified checking assertion with the IP vendor, the vendor may be able to speculate about the user's future plans--the IP user may be working on a new product that uses a wireless network with a different topology.
This information could be harmful if IP vendors disclose it to the IP user's competitors. 









==> figs/fsm.tex <==
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (31.7,-38) circle (3);
\draw (31.7,-38) node {$s'_0$};
\draw [black] (41.1,-28.1) circle (3);
\draw (41.1,-28.1) node {$s'_1$};
\draw [black] (55.6,-38) circle (3);
\draw (55.6,-38) node {$s'_2$};
\draw [black] (48.8,-38) circle (3);
\draw (48.8,-38) node {$s'_5$};
\draw [black] (56.8,-47.1) circle (3);
\draw (56.8,-47.1) node {$s'_3$};
\draw [black] (41.1,-47.1) circle (3);
\draw (41.1,-47.1) node {$s'_6$};
\draw [black] (41.1,-38) circle (3);
\draw (41.1,-38) node {$s'_4$};
\draw [black] (32.674,-35.169) arc (154.52702:118.44101:13.245);
\fill [black] (38.32,-29.22) -- (37.38,-29.16) -- (37.86,-30.04);
\draw [black] (43.959,-28.962) arc (63.51878:12.23119:8.863);
\fill [black] (48.67,-35.02) -- (48.99,-34.13) -- (48.01,-34.34);
\draw [black] (54.317,-40.705) arc (-31.66427:-84.1121:13.657);
\fill [black] (44.09,-47.12) -- (44.94,-47.54) -- (44.84,-46.54);
\draw [black] (57.485,-40.3) arc (26.07367:-11.04939:6.481);
\fill [black] (58.02,-44.39) -- (58.67,-43.7) -- (57.69,-43.51);
\draw [black] (53.816,-46.82) arc (-100.01125:-140.18345:18.494);
\fill [black] (42.83,-40.45) -- (42.95,-41.38) -- (43.72,-40.74);
\draw [black] (39.82,-35.304) arc (-164.67332:-195.32668:8.528);
\fill [black] (39.82,-30.8) -- (39.13,-31.44) -- (40.09,-31.7);
\draw [black] (48.15,-40.917) arc (-21.07065:-59.40207:10.093);
\fill [black] (43.87,-45.98) -- (44.81,-46) -- (44.3,-45.14);
\draw [black] (39.259,-44.776) arc (-156.81598:-203.18402:5.654);
\fill [black] (39.26,-40.32) -- (38.48,-40.86) -- (39.4,-41.26);
\draw [black] (38.33,-45.963) arc (-118.47019:-149.67173:13.983);
\fill [black] (32.93,-40.73) -- (32.9,-41.67) -- (33.76,-41.17);
\draw [black] (44.093,-28.069) arc (84.12816:27.22455:13.274);
\fill [black] (54.54,-35.2) -- (54.62,-34.26) -- (53.73,-34.72);
\draw [black] (24.5,-38) -- (28.7,-38);
\fill [black] (28.7,-38) -- (27.9,-37.5) -- (27.9,-38.5);
\end{tikzpicture}

==> figs/kripke.tex <==
\begin{tikzpicture}[scale=0.2]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (16.8,-26.1) circle (3);
\draw (16.8,-26.1) node {$(s'_0,0)$};
\draw [black] (37.3,-25.5) circle (3);
\draw (37.3,-25.5) node {$(s'_1,0)$};
\draw [black] (33.1,-43.3) circle (3);
\draw (33.1,-43.3) node {$(s'_2,0)$};
\draw [black] (42,-42.6) circle (3);
\draw (42,-42.6) node {$(s'_5,0)$};
\draw [black] (22.1,-43.3) circle (3);
\draw (22.1,-43.3) node {$(s'_3,0)$};
\draw [black] (26.5,-52.4) circle (3);
\draw (26.5,-52.4) node {$(s'_6,0)$};
\draw [black] (11.5,-38.1) circle (3);
\draw (11.5,-38.1) node {$(s'_4,0)$};
\draw [black] (28.9,-30.7) circle (3);
\draw (28.9,-30.7) node {$(s'_1,1)$};
\draw [black] (19.571,-24.954) arc (109.02447:74.32848:24.99);
\fill [black] (34.47,-24.52) -- (33.83,-23.82) -- (33.56,-24.78);
\draw [black] (8.9,-26.1) -- (13.8,-26.1);
\fill [black] (13.8,-26.1) -- (13,-25.6) -- (13,-26.6);
\draw [black] (39.232,-27.79) arc (35.37189:-4.63496:17.969);
\fill [black] (42.49,-39.64) -- (43.05,-38.89) -- (42.06,-38.81);
\draw [black] (38.248,-28.341) arc (12.74245:-39.29524:15.039);
\fill [black] (35.22,-41.18) -- (36.11,-40.88) -- (35.34,-40.25);
\draw [black] (30.677,-45.035) arc (-65.83193:-114.16807:7.516);
\fill [black] (24.52,-45.03) -- (25.05,-45.82) -- (25.46,-44.91);
\draw [black] (32.958,-46.28) arc (-13.30797:-58.59689:8.118);
\fill [black] (29.29,-51.34) -- (30.23,-51.35) -- (29.71,-50.5);
\draw [black] (19.113,-43.137) arc (-100.48645:-131.77555:11.679);
\fill [black] (13.46,-40.36) -- (13.72,-41.27) -- (14.39,-40.52);
\draw [black] (13.535,-35.9) arc (132.89526:93.18361:19.786);
\fill [black] (25.9,-30.64) -- (25.08,-30.18) -- (25.13,-31.18);
\draw [black] (41.168,-45.474) arc (-23.17772:-92.21538:12.228);
\fill [black] (29.45,-52.88) -- (30.23,-53.41) -- (30.27,-52.41);
\draw [black] (23.655,-51.456) arc (-112.41282:-154.85002:21.142);
\fill [black] (12.58,-40.9) -- (12.47,-41.83) -- (13.37,-41.41);
\draw [black] (18.961,-28.178) arc (43.16421:-2.67412:29.062);
\fill [black] (18.96,-28.18) -- (19.14,-29.1) -- (19.87,-28.42);
\draw [black] (31.018,-32.813) arc (37.86581:-0.99591:11.923);
\fill [black] (33.53,-40.34) -- (34.04,-39.55) -- (33.04,-39.53);
\draw [black] (31.76,-31.595) arc (67.80811:27.68806:17.873);
\fill [black] (40.83,-39.84) -- (40.91,-38.9) -- (40.02,-39.36);
\end{tikzpicture}

==> img/dimacs.tex <==

\begin{figure}
\begin{subfigure}[t]{0.45\columnwidth}
\begin{lstlisting}[style=dimcas,basicstyle=\ttfamily\scriptsize]
p cnf <@\textcolor{red}{32}@> 74 //ip design
-1 0
2 3 0
4 3 0
5 3 0
6 3 0
-2 -4 -5 -6 -3 0
...
26 -28 0
-26 28 0
29 0
30 0
-32 0
31 0
\end{lstlisting}
\caption{IP Design in CNF(DIMACS) generated by IP vendors}
\label{lst:cnfdesign}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\columnwidth}
\begin{lstlisting}[style=dimcas,basicstyle=\ttfamily\scriptsize]
p cnf 13 20 //ip user
<@\textcolor{red}{1}@> 0 
2 -3 0
4 2 0
3 -4 -2 0
2 0
...
3 -12 0
12 -3 0
4 -13 0
13 -4 0
-5 0
-8 0
-10 0
\end{lstlisting}
\caption{Assertion in CNF(DIMACS) generated by IP users}
\label{lst:cnfassertion_before}
\end{subfigure}
\begin{subfigure}[t]{0.45\columnwidth}
\begin{lstlisting}[style=dimcas,basicstyle=\ttfamily\scriptsize]
p cnf 13 20 //ip user - synced
<@\textcolor{red}{33}@> 0
34 -35 0
36 34 0
35 -36 -34 0
34 0
37 -21 0
...
25 -35 0
36 -27 0
27 -36 0
-37 0
-40 0
-42 0
\end{lstlisting}
\caption{IP users synchronize some integer identifier (e.g. values in red) to use the same namespace as that of the IP vendors}
\label{lst:cnfassertion_after}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.45\columnwidth}
\begin{lstlisting}[style=dimcas,basicstyle=\ttfamily\scriptsize]
p cnf 45 94 
//preamble is updated
-1 0
2 3 0
...
30 0
-32 0
31 0
33 0
34 -35 0
...
-37 0
-40 0
-42 0
\end{lstlisting}
\caption{\texttt{hw-ppSAT} accept input from IP users and IP vendors to check \textit{SAT/UNSAT}}
\label{lst:cnfppsat}
\end{subfigure}
\caption{CNF generated by IP users and IP vendors for jointly verifying IP design against assertion}
\end{figure}



==> img/dynamicindex.tex <==
    \begin{tikzpicture}
        \def\verilog{
            \lstinline[style=vcode]{module mux(}/0,%
            \lstinline[style=vcode]{input [1:0] ins,}/2,%
            \lstinline[style=vcode]{input select,}/2,%
            \lstinline[style=vcode]{output mux_out);}/2,%
            \lstinline[style=vcode]{assign mux_out = ins[select];}/1,%
            \lstinline[style=vcode]{endmodule}/0%
        }
        \foreach \txt\offset [count=\y from 0] in \verilog {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (vcode\y) at (1ex*\offset, -0.3*\y) {\txt};
        }
        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(vcode0.north west) in let \p2=(vcode5.south east) in
            (vcode0.north west) rectangle (\x1 + 2.1in, \y2);
            \node[
                anchor=south west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (header) at(vcode0.north west) {2-1 multiplexer};
            \draw let \p2=(header.north west) in let \p1=(vcode0.north west) in
                (vcode0.north west) |- (\x1 + 1.3in, \y2)
                    -- (\x1 + 1.35in, \y1);
        \end{scope}

        \def\formalcode{
            \lstinline[style=hwscm]{mux.mux_out\#0 <--}/0,%
            \lstinline[style=hwscm]{If(0 == mux.select\#0,}/1,%
            \lstinline[style=hwscm]{Extract(0, 0, mux.ins\#0),}/2,%
            \lstinline[style=hwscm]{Extract(1, 1, mux.ins\#0))}/2%
        }
        \foreach \txt\offset [count=\y from 0] in \formalcode {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (hwscm\y) at(1ex*\offset+1.25in, -0.3*\y - 1.75) {\txt};
        }

        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(hwscm0.north west) in
                let \p2=(hwscm3.south east) in
                (\x1, \y1) rectangle (\x1 + 2.1in, \y2);
            \path let \p1=(hwscm3.south west) in let \p2=(hwscm0.north west) in
                node[coordinate] (headerpos) at(\x2, \y1) {};
            \node[
                anchor=north west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (scmheader) at(headerpos) {SCM representation};
            \draw let \p1=(scmheader.south west) in let \p2=(scmheader.north west) in
                (\x2, \y2) |- (\x2 + 1.3in, \y1)
                    -- (\x2 + 1.35in, \y2);
        \end{scope}

        \node[coordinate, font=\ttfamily\footnotesize] (arrowtgt)
            at ($(hwscm1.south west) - (1ex, 0)$) {};
        \draw[thick, red, -latex']
            (vcode5) |- (arrowtgt);
    \end{tikzpicture}
    
    % \caption{Dynamic indexing transformation.}
    % \label{fig:dynamic_indexing}


==> img/implicitelse.tex <==
 \begin{tikzpicture}
        \def\verilog{
            \lstinline[style=vcode]{always @(posedge clk)}/0,%
            \lstinline[style=vcode]{if(rst)}/1,%
            \lstinline[style=vcode]{result <= 1'b0;}/2,%
            \lstinline[style=vcode]{else if(control)}/1,%
            \lstinline[style=vcode]{result <= 1'b1;}/2%
        }
        \foreach \txt\offset [count=\y from 0] in \verilog {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (vcode\y) at (1ex*\offset, -0.3*\y) {\txt};
        }
        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(vcode0.north west) in let \p2=(vcode4.south east) in
            (vcode0.north west) rectangle (\x1 + 2.1in, \y2);
            \node[
                anchor=south west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (header) at(vcode0.north west) {implicit};
            \draw let \p2=(header.north west) in let \p1=(vcode0.north west) in
                (vcode0.north west) |- (\x1 + 1.3in, \y2)
                    -- (\x1 + 1.35in, \y1);
        \end{scope}

        \def\formalcode{
            \lstinline[style=hwscm]{implicit.result\#0 <--}/0,%
            \lstinline[style=hwscm]{If(implicit.rst\#-1 == 1,}/1,%
            \lstinline[style=hwscm]{0,}/2,%
            \lstinline[style=hwscm]{If(implicit.control\#-1 == 1,}/2,%
            \lstinline[style=hwscm]{1,}/3,%
            \lstinline[style=hwscm]{implicit.result\#-1))}/3%
        }
        \foreach \txt\offset [count=\y from 0] in \formalcode {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (hwscm\y) at(1ex*\offset+1.25in, -0.3*\y - 0.5) {\txt};
        }

        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(hwscm0.north west) in
                let \p2=(hwscm5.south east) in
                (\x1, \y1) rectangle (\x1 + 2.1in, \y2);
            \path let \p1=(hwscm5.south west) in let \p2=(hwscm0.north west) in
                node[coordinate] (headerpos) at(\x2, \y1) {};
            \node[
                anchor=north west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (scmheader) at(headerpos) {SCM representation};
            \draw let \p1=(scmheader.south west) in let \p2=(scmheader.north west) in
                (\x2, \y2) |- (\x2 + 1.3in, \y1)
                    -- (\x2 + 1.35in, \y2);
        \end{scope}

        \node[font=\ttfamily\footnotesize] (arrowtgt)
            at ($(hwscm4.south west) - (2ex, 0)$) {};
        \draw[thick, red, -latex']
            (vcode4) |- (arrowtgt);
    \end{tikzpicture}
    
    % \caption{Implicit \lstinline[style=vcode]{else} transformation.}
    % \label{fig:implicitelse}


==> img/multicycle.tex <==
    \begin{tikzpicture}
        \def\verilog{
            \lstinline[style=vcode]{module counter(}/0,%
            \lstinline[style=vcode]{input wire clk, rst,}/2,%
            \lstinline[style=vcode]{output reg [7:0] ctr);}/2,%
            \lstinline[style=vcode]{always @posedge(clk)}/1,
            \lstinline[style=vcode]{if(rst) ctr <= 8'b0;}/2,
            \lstinline[style=vcode]{else ctr = ctr + 8'b1;}/2,
            \lstinline[style=vcode]{endmodule}/0%
        }
        \foreach \txt\offset [count=\y from 0] in \verilog {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (vcode\y) at (1ex*\offset, -0.3*\y) {\txt};
        }
        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(vcode0.north west) in let \p2=(vcode6.south east) in
            (vcode0.north west) rectangle (\x1 + 2.1in, \y2);
            \node[
                anchor=south west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (header) at(vcode0.north west) {Counter circuit};
            \draw let \p2=(header.north west) in let \p1=(vcode0.north west) in
                (vcode0.north west) |- (\x1 + 1.3in, \y2)
                    -- (\x1 + 1.35in, \y1);
        \end{scope}

        \def\formalcode{
            \lstinline[style=hwscm]{counter.ctr\#0 <--}/0,%
            \lstinline[style=hwscm]{If(1 == counter.rst\#-1,}/1,%
            \lstinline[style=hwscm]{0,}/2,%
            \lstinline[style=hwscm]{counter.ctr\#-1 + 1)}/2,%
            \lstinline[style=hwscm]{counter.ctr\#-1 <--}/0,%
            \lstinline[style=hwscm]{If(1 == counter.rst\#-2),}/1,%
            \lstinline[style=hwscm]{0,}/2,
            \lstinline[style=hwscm]{counter.ctr\#-2 + 1)}/2,%
            \lstinline[style=hwscm]{counter.ctr\#-2 <--}/0,
            \lstinline[style=hwscm]{...}/1%
        }
        \foreach \txt\offset [count=\y from 0] in \formalcode {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (hwscm\y) at(1ex*\offset+1.25in, -0.3*\y - 2) {\txt};
        }

        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(hwscm0.north west) in
                let \p2=(hwscm9.south east) in
                (\x1, \y1) rectangle (\x1 + 2.1in, \y2);
            \path let \p1=(hwscm9.south west) in let \p2=(hwscm0.north west) in
                node[coordinate] (headerpos) at(\x2, \y1) {};
            \node[
                anchor=north west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (scmheader) at(headerpos) {SCM representation};
            \draw let \p1=(scmheader.south west) in let \p2=(scmheader.north west) in
                (\x2, \y2) |- (\x2 + 1.3in, \y1)
                    -- (\x2 + 1.35in, \y2);
        \end{scope}

        \node[font=\ttfamily\footnotesize] (arrowtgt)
            at ($(hwscm4.south west) - (-1ex, 0)$) {};
        \draw[thick, red, -latex']
            (vcode6) |- (arrowtgt);
    \end{tikzpicture}
    
    % \caption{Multicycle sequential circuits.}
    % \label{fig:circuit_sequential}


==> img/twoDarray.tex <==
    \begin{tikzpicture}
        \def\verilog{
            \lstinline[style=vcode]{module rom_table(}/0,%
            \lstinline[style=vcode]{input wire [1:0] addr,}/2,%
            \lstinline[style=vcode]{output wire [3:0] data);}/2,%
            \lstinline[style=vcode]{reg [3:0] store [0:3];}/1,%
            \lstinline[style=vcode]{initial}/1,
            \lstinline[style=vcode]{$readmemb("datatable.vhi",}/2,
            \lstinline[style=vcode]{store);}/14,
            \lstinline[style=vcode]{assign data = store[select];}/1,
            \lstinline[style=vcode]{endmodule}/0%
        }
        \foreach \txt\offset [count=\y from 0] in \verilog {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (vcode\y) at (1ex*\offset, -0.3*\y) {\txt};
        }
        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(vcode0.north west) in let \p2=(vcode8.south east) in
            (vcode0.north west) rectangle (\x1 + 2.1in, \y2);
            \node[
                anchor=south west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (header) at(vcode0.north west) {ROM Implementation};
            \draw let \p2=(header.north west) in let \p1=(vcode0.north west) in
                (vcode0.north west) |- (\x1 + 1.3in, \y2)
                    -- (\x1 + 1.35in, \y1);
        \end{scope}

        \def\formalcode{
            \lstinline[style=hwscm]{rom_table.data\#0 <--}/0,%
            \lstinline[style=hwscm]{If(0 == rom_table.addr\#0,}/1,%
            \lstinline[style=hwscm]{rom_table.store_index_0\#0,}/2,%
            \lstinline[style=hwscm]{If(1 == rom_table.addr\#0,}/2,%
            \lstinline[style=hwscm]{rom_table.store_index_1\#0,}/3,%
            \lstinline[style=hwscm]{...}/3,%
            \lstinline[style=hwscm]{rom_table.store_index_0\#0 <--}/0,
            \lstinline[style=hwscm]{file_read_value_0}/1,%
            \lstinline[style=hwscm]{rom_table.store_index_1\#0 <--}/0,
            \lstinline[style=hwscm]{file_read_value_1}/1,%
            \lstinline[style=hwscm]{...}/0%
        }
        \foreach \txt\offset [count=\y from 0] in \formalcode {
            \node[
                anchor=west,
                font=\ttfamily\footnotesize,
            ] (hwscm\y) at(1ex*\offset+1.25in, -0.3*\y - 2.55) {\txt};
        }

        \begin{scope}[on background layer]
            \draw[fill=gray!10] let \p1=(hwscm0.north west) in
                let \p2=(hwscm10.south east) in
                (\x1, \y1) rectangle (\x1 + 2.1in, \y2);
            \path let \p1=(hwscm10.south west) in let \p2=(hwscm0.north west) in
                node[coordinate] (headerpos) at(\x2, \y1) {};
            \node[
                anchor=north west,
                font=\ttfamily\footnotesize,
                color=blue,
            ] (scmheader) at(headerpos) {SCM representation};
            \draw let \p1=(scmheader.south west) in let \p2=(scmheader.north west) in
                (\x2, \y2) |- (\x2 + 1.3in, \y1)
                    -- (\x2 + 1.35in, \y2);
        \end{scope}

        \node[font=\ttfamily\footnotesize] (arrowtgt)
            at ($(hwscm4.south west) - (2ex, 0)$) {};
        \draw[thick, red, -latex']
            (vcode8) |- (arrowtgt);
    \end{tikzpicture}
    
    % \caption{Resolution of 2D array indexing.}
    % \label{fig:arrayselection}


==> revision/Crypto_overhead.tex <==



\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
       \includegraphics[width=\linewidth]{figs/ot_vs_mn_depth1-5_mb_nomn_style_big.pdf}
        \caption*{Fig.~\ref{fig:ot_vs_design}:\answer{Communication overhead of the $1$-out-of-$2^{\textit{depth}}$ OT protocol versus design size ($n_{var}\times n_{cls}$). Each point represents a benchmark instance. The overhead scales approximately linearly with design size and increases with portfolio size $2^{\textit{depth}}$.}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/one_step_overhead_style.pdf}
        \caption*{Fig.~\ref{fig:overhead_all}:\answer{ 2PC communication overhead per giant step measured by the garbled circuit size. The circuit size grows approximately linearly with the design size ($n_{var}\times n_{cls}$)}}
    \end{subfigure}
\end{figure}


Figure~\ref{fig:ot_vs_design} illustrates the communication overhead introduced by the $1$-out-of-$2^{\textit{depth}}$ OT protocol. 
The x-axis represents the design size measured as the product of the number of variables and clauses ($n_{var}\times n_{cls}$), while the y-axis reports the total OT cost in MB. Each point corresponds to a verification instance.
As shown in the Figure~\ref{fig:ot_vs_design}, the OT communication overhead increases approximately linearly with the design size. As discussed in Section~\ref{subsec:overviewppsat}, each clause in the CNF-encoded design is represented as a pair of binary vectors of length $n$. Consequently, the OT overhead scales with $n_{var} \times n_{cls}$.

Furthermore, the OT overhead grows approximately linearly with $2^{\textit{depth}}$. In a $1$-out-of-$2^{\textit{depth}}$ OT protocol, increasing $\textit{depth}$ enlarges the portfolio size $N = 2^{\textit{depth}}$. As a result, more masked candidate messages must be communicated during the transfer. For the smallest benchmark, \texttt{b02}, with $\textit{depth}=1$, the OT communication overhead is approximately 0.022~MB, whereas for the largest benchmark, \texttt{mem\_ctrl}, with $\textit{depth}=5$, the OT overhead reaches approximately 517~MB.

Figure~\ref{fig:overhead_all} shows the cryptographic overhead of 2PC. This overhead primarily arises from \texttt{hw-ppSAT}, which adapts the DPLL algorithm as its core routine and compiles each \textit{giant step} into the garbled circuit, where the communication overhead scales linearly with the number of AND gates (about 32 bytes per gate). Thus, the total communication cost is the per-step circuit cost multiplied by the number of \textit{giant steps}.
Similar to the OT protocol, the circuit size grows approximately linearly with the design size. Larger designs produce larger CNF encodings and require more evaluation during verification. For the largest design, \texttt{mem\_ctrl}, the circuit size can reach around 3 billion gates per step, making secure verification impractical without optimization. After applying design pruning, we reduce the communication overhead to about 6 million gates per step. Furthermore, using the control-flow-guided heuristic, the number of giant steps is reduced from more than 20,000 to 236, making secure verification feasible.


==> revision/assertion_signal.tex <==
We acknowledge that repeated verification queries may enable property probing. To handle this concern, practical deployments should enforce query limits or auditing mechanisms. As discussed in Section~\ref{subsec:preprocess}, the IP vendor exposes only a \emph{public semantic map} that allows users to construct verification properties. The variables appearing in this semantic map represent only a subset of the entire design variables, which restricts the information that can be inferred through property probing.

To better understand the potential leakage surface, we empirically analyze the proportion of variables used in assertions across all benchmarks. As shown in Figure~\ref{fig:assertion_signal}, the average percentage of design variables referenced in verification properties is 2.49\%. The maximum case occurs in \texttt{wb\_conmax\_T300\_prune}, where the assertion involves 25.68\% of the design variables. These results suggest that even if a user attempts to perform property probing by repeatedly modifying the assertion variables, the observable portion of the design behavior remains limited to a relatively small subset of the overall design.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/assertion_used_over_design_pct.pdf}
    \caption*{Fig.~\ref{fig:assertion_signal}:\answer{ Percentage of design variables referenced by verification assertions relative to the total number of design variables across all benchmarks. The results show that verification properties typically involve only a small subset of the design variables (2.49\% on average).}}
\end{figure}


==> revision/decoy_strategy.tex <==
Firstly, design pruning in \tool is an optional optimization introduced to improve efficiency for large designs. When desired, the protocol can directly proceed to oblivious design selection and secure verification without pruning.
Secondly, as discussed in Section~\ref{subsec:prune}, pruning requires revealing the property signal to the vendor for COI dependency analysis. However, this disclosure is limited: only the signal identifier is revealed, while the semantics of the property remain private to the user.

To further mitigate potential side-channel leakage, users could first submit pruning requests for multiple candidate designs as decoys to obscure the actual verification target, and then proceed with verification for the selected design. The overhead is mainly from the preprocessing step locally performed by the vendor, and there is no additional overhead to the subsequent oblivious design selection and secure verification phases. 

==> revision/design_pruning.tex <==
Design pruning is inherently based on cone-of-influence (COI) reduction. \input{revision/COI} When the verification property involves only a localized portion of the design, design pruning significantly reduces the number of variables and clauses in the encoded formula, leading to substantial reductions in both SAT solving time and cryptographic overhead. For instance, large IP modules with multiple control and data paths (e.g., \texttt{memctrl\_T100} and \texttt{RS232\_T700}) exhibit orders-of-magnitude improvements after pruning. In contrast, compact single-purpose designs with tightly coupled logic (e.g., small FSM benchmarks such as \texttt{b02\_2} and \texttt{Rrobin}) show little to no benefit, since most of the circuit remains within the cone of influence of the property.

==> revision/flatten_netlist.tex <==
We clarify that \tool can support formal verification on flattened netlists, as during the IP translation stage (Section~\ref{subsec:preprocess}), the hardware design is eventually translated into CNF, which can be constructed directly from gate-level netlist representations. The property can also be compiled into the circuit~\cite {finkbeiner2015algorithms}. Meanwhile, \texttt{hw-ppSAT} remains applicable in such scenarios as long as a Cone of Influence (COI) reduction or control-flow dependency exists. However, we do not generally recommend this practice.

First, \tool is primarily designed to protect the confidentiality of assertion-based formal verification, where verification properties are typically derived from behavioral-level abstractions. In contrast, flattened gate-level netlists often lack the semantic information necessary to meaningfully express such properties. Second, synthesis binds the design to a particular cell library. In many cases, complex operators (e.g., multiplexers) must be decomposed into multiple primitive gates such as AND and NOT gates. This transformation introduces additional auxiliary variables during CNF generation and significantly increases the number of clauses and variables. Since \tool encodes the CNF using a pair of binary matrices (as discussed in Section~\ref{subsec:overviewppsat}), the resulting increase in CNF size can substantially amplify both the computational overhead of the 2PC protocol~\cite{luo2022ppsat} and the communication overhead discussed in Section~\ref{subsec:overhead}. 

==> revision/heuristic_set.tex <==
To prevent information leakage, the heuristic set associated with each IP design is retrieved through the same Oblivious Design Selection protocol described in Section~\ref{subsec:ot_selection}. Concretely, the IP vendor generates a heuristic set $\heuset^k$ for each design $\phi_k$ during preprocessing and includes it in the message vector used in the OT protocol. The IP user then retrieves the heuristic corresponding to the selected design using a 1-out-of-$N$ OT invocation
$$
(\heuset^i, \bot) \leftarrow {\sf OT}(i, \{\heuset^1, \heuset^2, \ldots, \heuset^N\}).
$$
By the security guarantee of OT, the user learns only $\heuset^i$ and obtains no information about $\{\heuset^j\}_{j\ne i}$, while the vendor learns nothing about the user's selection $i$. Furthermore, since $\heuset$ only specifies a partial ordering of variables for branching decisions, it does not reveal structural information about the underlying circuit. 
We further quantify the overhead of the OT-based heuristic retrieval in Figure~\ref{fig:heuristic_count}. 

Among all benchmarks, \texttt{adbg} has the largest heuristic set, containing 308 literals. 
Even with a 128-bit encoding per literal, the total communication cost is approximately 4.8~KB, therefore the communication overhead introduced by retrieving $\heuset$ via OT is negligible compared to the design selection and verification phases in Section~\ref{subsec:overhead}.



==> revision/mask_freshness.tex <==

If the same masking randomness were reused across different verification
sessions, colluding users could correlate masked artifacts obtained from
multiple queries and infer structural relationships between protected
designs. Recall that each design $\phi_k$ is represented as a pair of binary
matrices $(P_k,N_k)$. If two masked instances are generated using the
same masking matrices $(R_P,R_N)$, i.e.,
\[
(\widetilde P_k^{(1)},\widetilde N_k^{(1)})
=
(P_k^{(1)}\oplus R_P,\;N_k^{(1)}\oplus R_N),
\]
\[
(\widetilde P_k^{(2)},\widetilde N_k^{(2)})
=
(P_k^{(2)}\oplus R_P,\;N_k^{(2)}\oplus R_N),
\]
Colluding users could eliminate the masks by computing
\[
(\widetilde P_k^{(1)},\widetilde N_k^{(1)})
\oplus
(\widetilde P_k^{(2)},\widetilde N_k^{(2)})
=
(P_k^{(1)}\oplus P_k^{(2)},\;
 N_k^{(1)}\oplus N_k^{(2)}),
\]



==> revision/non_ppsat.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/benchmark_plain_modified_oneplot_single_mark.pdf}
    \caption*{Fig.~\ref{fig:nonppSAT}: \answer{Runtime of the non-private baseline implementation of \texttt{hw-ppSAT} without 2PC. The results indicate that solver runtime is largely dominated by the number of executed steps.}}
\end{figure}

We implement \texttt{hw-ppSAT} and \texttt{ppSAT} in Python and include the non-private baseline experiment in Figure~\ref{fig:nonppSAT}. To ensure consistency with Table~\ref{tab:exp}, the timeout is set to 20,000 giant steps, identical to that used in Table~\ref{tab:exp}. Figure~\ref{fig:nonppSAT} shows that reaching 20,000 giant steps corresponds to approximately 100 seconds for the largest timed-out design. The results also indicate that solver runtime is largely dominated by the number of executed giant steps, as the baseline implementations follow the same DPLL core routine.
The most time-consuming benchmark, \texttt{memctrl\_T100}, finishes verification in 37.9 seconds, corresponding to an approximately $8.4 \times 10^{4}$ slowdown compared with the non-private baseline. In contrast, \texttt{b02\_1\_prune} finishes within 0.02 seconds, incurring an overhead of about $3 \times 10^{3}$. As expected, the non-private verification implementation is significantly faster than the privacy-preserving one due to the additional cryptographic operations. Moreover, the slowdown is not uniform across benchmarks and primarily depends on the design size, as larger designs incur substantially higher overhead in GC-based 2PC computation.

==> revision/pratical_challenge.tex <==
\tool is designed to operate as a lightweight preprocessing and verification layer on top of existing verification flows rather than replacing them. In practice, hardware designs written in synthesizable RTL are first processed by a static-analysis frontend that performs dataflow analysis. The design is then translated into an SMT representation and subsequently converted into CNF using standard solver infrastructure, following the standard SAT-based hardware verification pipeline.

\texttt{hw-ppSAT} serves as the checker that enables privacy-preserving formal verification. Although current commercial formal verification tools do not natively support such capabilities, the proposed framework can be integrated as an additional execution engine in verification tools such as VC Formal~\cite{synopsys:vcug} or JasperGold~\cite{JasperGold}.

We also revised the Section~\ref{sec:con} to declare the potential challenges of integrating \tool in the existing verification workflow as follows.

\revise{A practical challenge of \tool is its interactive protocol, where stages such as oblivious design selection and secure SAT solving require synchronized message exchanges between the IP vendor and the IP user, introducing additional latency compared with offline verification. Despite this overhead, the framework remains compatible with existing post-licensing IP protection solutions and can be deployed within current hardware supply-chain ecosystems.}

We believe this requirement is consistent with typical secure computation protocols and does not fundamentally hinder practical deployment. In realistic IP trading scenarios, verification is usually performed once before the transaction is finalized, and both parties can schedule the protocol execution in a controlled environment with stable connectivity. Moreover, many steps in the protocol can be pipelined or parallelized, and the communication overhead is largely dominated by the SAT-solving phase, which is already the primary computational bottleneck in privacy-preserving verification.


\input{revision/scalability}

==> revision/repeated_query.tex <==
Property probing through repeated queries can introduce potential leakage.
The sequence of $\textsf{SAT}/\textsf{UNSAT}$ outcomes may act as a behavioral oracle, which could allow adversaries to infer the behavioral information of the design. However, as discussed in Section~\ref{subsec:preprocess}, BlindMarket restricts verification properties to a predefined set of signals derived from the public semantic map. This restriction limits an adversary’s ability to construct arbitrary probing properties and thereby significantly reduces the feasibility of large-scale reverse engineering of the hidden design structure.

==> revision/scalability.tex <==
We admit that the current workflow is not intended for large-scale SoC verification. This limitation stems from both the intrinsic complexity of formal verification~\cite{grimm2018survey} and the overhead introduced by cryptographic protocols~\cite{luo2022ppsat}. In particular, the communication and computation costs of 2PC scale with the size of the garbled circuit, as secure computation evaluates the circuit gate by gate (Section~\ref{subsec:overhead}).
Meanwhile, the existing approaches do not adequately address this issue. Prior work~\cite{mouris2020pythia,mouris2023mploc} primarily targets small benchmark circuits such as ISCAS’85 and relies on simulation-based approaches. In contrast, our framework supports designs of similar scale while providing formal verification guarantees, and is suitable for larger IP-level verification tasks as demonstrated in Section~\ref{tab:source}. Furthermore, many industrial verification tasks can naturally be modularized at the IP level, which aligns well with the intended deployment scenario of our framework. Importantly, this limitation does not preclude industrial applicability. In practice, formal verification commonly relies on abstraction to manage complexity. When detailed design behavior must remain confidential, designers can construct abstract models~\cite{biere2009handbook} for subsequent verification. Our goal is therefore not to replace full-chip verification, but to enable privacy-preserving formal verification for IP-level modules where confidentiality is critical.

==> revision/trade_off.tex <==
We agree that there is a trade-off between verification speed and IP confidentiality when applying design pruning in real-world deployment scenarios. When the IP user is willing to disclose the set of assertion-related signals to the IP vendor, the vendor can perform cone-of-influence (COI) reduction to remove irrelevant logic before secure verification. This pruning step reduces the size of the resulting SAT instance and significantly improves verification speed, as shown in Table~\ref{tab:exp}. Importantly, this limited disclosure does not reveal the implementation details of the IP design. To further mitigate potential leakage, we also introduce a decoy-based strategy during design pruning.
Additionally, the proposed \texttt{hw-ppSAT} does not affect solver completeness and incurs negligible communication overhead, as it only influences the branching order during the SAT solving process.

We revised the corresponding mitigation in Section~\ref{subsec:prune} as follows.

\revise{Pruning is performed offline on the vendor side based on the user-provided property signal. Although the semantics of the property remain private to the user, the signal itself must be revealed to the vendor for COI analysis. To mitigate this disclosure, users may first submit pruning requests for multiple candidate designs as decoys to hide the actual verification target and then proceed with verification for the selected design.}






==> sections/benchmarkdetails.tex <==
% \input{sections/benchmark}
% \subsection{Experiment.}\label{ap:bench}
% \subsubsection{Benchmark Setup}
% Table~\ref{tab:source} lists all benchmark descriptions and detailed assertions.
% We verify the bounded \textit{assert property} and \textit{cover property} on ANSI-C~\cite{mtk2016}, Opencore~\cite{opencores} and Trusthub~\cite{TrustHub}. ANSI includes the corresponding assertions within the code, and Trusthub, where chip-level designs
% are annotated with known vulnerabilities that can be expressed as \textit{cover property}.
% For example, we verify constraints on output signals and state transitions to ensure correct sequential behaviour in the finite state machines \texttt{b01} and \texttt{b02}. The \texttt{Rrobin} design serves as a round-robin arbiter, where mutual exclusion is enforced by asserting that two acknowledge outputs should never be high simultaneously. The \texttt{adbg} module, a JTAG-compliant TAP controller, includes a password check mechanism, and we verify that no invalid input can bypass this check to set \texttt{passchk = 1}. In the Trusthub benchmark, \texttt{RS232\_T700} verifies whether an input sequence causes the transmitter to enter a Denial-of-Service (DoS) state. In \texttt{memctrl\_T100}, we check whether writing \texttt{0x77} in the CSR register results in the flash sleep bit (\texttt{fs}) being erroneously set to 1. Lastly, \texttt{wb\_conmax\_T300} checks whether any crafted input pattern allows a master to alter its destination slave unexpectedly.

% \subsubsection{Oblivious IP Selection}\label{ap:oblivousipselect}


==> sections/discussion.tex <==

\section{Discussion and Future Work}\label{sec:df}

% \xiaolong{PPMC enhancement - Time/scale}

%hmm I prefer to skip this part other wise I would repeat what Samuel said in his paper... Like 1) symbolic model checking 2) include CTL^* in the ppmc 

% \xiaolong{Auto parser}

% We consider the following directions as our future work.
% \begin{enumerate}
%      \item Our zero trust verification framework is limited to performing formal verification of functional and security properties. We will consider expanding its functionality to include timing analysis and simulation. 
%   % \item Our Zero trust verification framework relies on the PPMC protocol to check properties. The IP User and the IP Vendor need to translate their models locally to meet the requirement of the PPMC protocol. We consider migrating automatic translation into our existing framework in the future.
%     \item Currently, we manually translate from natural language specifications to CTL formula. We plan to automate this process by developing a parser which can translate wide variety of SystemVerilog and PSL assertions.
    
%     \item The Kripke structure conversion is limited to soft IP cores with FSM. We will further investigate to expand our framework's capability to read firm IP cores and any general IP design. 
% \end{enumerate}





% remain uncertainty : cannot do 1 to 1 map for each assertion to CTL formula 


==> sections/experiment_setup.tex <==
\begin{table*}[!h]
    \begin{center}
    % \resizebox{0.5\columnwidth}{!}{
%ZedBoard Zynq Evaluation and Development Kit (xc7z020clg484-1)
    %\begin{tabularx}{\textwidth}{ ccccccX }
    \begin{tabularx}{\textwidth}{ cccX }
    \toprule
  \textbf{RTL}   &\textbf{FF}&\textbf{LUT} &\textbf{Property in SVA} \\ %\hline
    \midrule[0.5\lightrulewidth]
    b01
    &%benchmark

    5
    &%FF
    5
    &%LUT
    \lstinline[style=vcode]{assert property (OVERFLW==1 |-> ##2 (OVERFLW==0))}
    %property
    \\

     b02-1
    &%benchmark

    4
    &%FF
    3
    &%LUT
   \lstinline[style=vcode]{assert property (stato==D |-> ##2 (stato==B))}
    %property
    \\

    b02-2
    &%benchmark

    4
    &%FF
    3
    &%LUT
   \lstinline[style=vcode]{assert property (U==1 |-> ##1 U==0)}
    %property
    \\

    b02-3
    &%benchmark

    4
    &%FF
    3
    &%LUT
   \lstinline[style=vcode]{assert property (U==1 |-> stato==B)}
    %property
    \\

    b03
    &%benchmark

    31
    &%FF
    18
    &%LUT
   \lstinline[style=vcode]{assert property (GRANT_O==0 || GRANT_O==8 || GRANT_O==4 || GRANT_O==2 || GRANT_O==1)}
    %property
    \\

    Rrobin
    &%benchmark

    5
    &%FF
    3
    &%LUT
 \lstinline[style=vcode]{assert property (ack0==0 || ack1==0)}
    %property
    \\

    Prep3
    &%benchmark
    16
    &%FF
    17
    &%LUT
\lstinline[style=vcode]{assert property (next_out == 8'h20 |-> ##1 (next_out == 8'h11 || next_out = 8'h30 ))}
    %property
    \\

    RS232-T700
    &%benchmark
    26
    &%FF
    43
    &%LUT
\lstinline[style=vcode]{cover property (state_DataSend==7)}
    %property
    \\

%     lock\_case
%     &%benchmark
%     2
%     &%FF
%     7
%     &%LUT
% \lstinline[style=vcode]{cover property (unlocked==1)}
%     %property
%     \\




    \bottomrule  
    \end{tabularx}
    % }
    \end{center}
        \caption{Experimental Setup: RTL (as would be provided by IP vendors) and properties in SVA (as would be provided by IP users).\liu{assertion could be used by xx \cite{}}\ning{table index type}} \label{tab:expsetup}

\end{table*}                                        

==> sections/heuristic.tex <==
\begin{table*}[!h]
    \begin{center}
    % \resizebox{0.5\columnwidth}{!}{
%ZedBoard Zynq Evaluation and Development Kit (xc7z020clg484-1)
    %\begin{tabularx}{\textwidth}{ ccccccX }
    \begin{tabularx}{\textwidth}{ ccccc }
    \toprule
  \textbf{RTL}   &\textbf{DLIS}&\textbf{Weighted-RAND} &\textbf{RAND} &\textbf{HW-DLIS}\\ %\hline
    \midrule[0.5\lightrulewidth]
b01&
 38m45.706s &%det_freq
Stack full&% weight_random
1m33.186s&%rand
38m34.620s%hardware
\\
b02-1&
0m21.175s&%det_freq 105 round
0m39.206s &% weight_random 105 round
6m39.326s&%rand 1266 round
0m20.958s %hardware 105 round
\\
b02-2&
14m52.081s&%det_freq
2m1.906s&% weight_random
Stack Full&%rand
14m51.292s%hardware
\\
b02-3&
0m6.106s&%det_freq 159 round
0m8.089s&% weight_random 116 round
0m3.473s&%rand 119 round
0m6.141s%hardware 159 round
\\
b03&
0m23.219s&%det_freq  60 round
0m41.435s &% weight_random 60 round
0m15.792s &%rand 60 rounds
0m23.703s %hardware 60 round
\\
lock&
0m16.877s&%det_freq 142 round
Stack Full&% weight_random
&%rand
0m16.880s%hardware 142 round
\\








    \bottomrule  
    \end{tabularx}
    % }
    \end{center}
        \caption{Experiment Setup: RTL provided by IP vendors and Property in SVA provided by IP users} 
\end{table*}                                        

==> sections/motivating_example.tex <==
\section{Motivating Example}\label{sec:motivate}
%automation in agriculture
%microcontroller-based automation
% exposed API for multiple sensors
%ADC module: analog sensors /Temperature/ Pressure
%serial communication protocol spi/i2c/uart /Digital Sensors /Accelerometer, Gyroscope
% built-in Bluetooth / Wi-Fi capabilities
%Arduino
%calculations
%Microcontroller-based automation systems are rapidly growing in various traditional low-tech fields\cite{nourizadeh2009medical,asadullah2016overview,edan2009automation}. 
% including healthcare\cite{nourizadeh2009medical}, home automation\cite{asadullah2016overview}, and agriculture\cite{edan2009automation}. Various companies provide tailored services via embedded automation systems to their customers.
\noindent Fabless companies, as IP users, often prioritize economies of scale and typically do not procure IP with varying specifications from vendors for different product lines. Instead, they often acquire COTS IP and then customize its usage as they require. This can lead to under-utilization of the functionalities offered by the IP vendors. For instance, Apple utilizes only a fraction of the available memory from RAM IP in its latest iPad models~\cite{macrumors2024}. Similarly, Tesla has chosen to restrict access to features such as heated seats behind a paywall~\cite{motor1_tesla_2024}. Therefore, the IP verification phase could possibly take place on just the subset of the IP interfaces intended for use.

% ranging from serial communication ports, ADC modules, to Bluetooth modules and Wi-Fi modules. However, not every interface sees practical use. For example, units used for data collection often do not require wireless communication features, while those tasked with data processing often do not interact with sensors.


% In precision agriculture, services for real-time crop health monitoring, yields, and storage are achieved by leveraging multi-level embedded hardware, including microcontrollers, sensors, and communication networks~\cite{edan2009automation}. The functionalities of a specialized system are achieved by integrating various hardware components that are IP designs and sold by IP vendors. 
% receive service on continuously monitoring crop health, yields, and storage in real time, receive instant alerts, and predict future needs. 
% Such systems optimize grain quality, prevent spoilage, and reduce energy costs.
% These benefits stem from the integrated use of multi-level embedded hardware, including microcontrollers, sensors, and communication networks, which work together to collect, transmit, compute, and analyze data.
% Most agritech companies offer tailored service 
% offering tailored services by integrating COTS IPs sold by other IP vendors,
% typically don't specialize in chip customization. Instead, they prefer to integrate COTS IPs. 
%
% NXP LPC 802 \cite{NXP_LPC802_UM}
%Wireless Mesh Networking: An IoT-Oriented Perspective Survey on Relevant Technologies
%is a microcontroller similar to the ESP32 \cite{esp32refmanual}. It
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.75\columnwidth]{figs/motivating2.png}
%     \caption{To advance its new business model, the Agritech company (the IP user) seeks to verify the WiFi interface of the IP before purchasing it from the Microcontroller Developer (the IP vendor). The Microcontroller Developer wants to protect its designs, while the Agritech company wants to protect its assertions. \tool can be used to meet the requirements of both parties.}
%     % \ning{TODO: explaination with a little bit more details and with generalization. Like instead solely Agritech company use "Agritech company (IP users)". concretize  "completing the business contract" by "Agritech company (IP user)  want to buy XXX' XXX"}}
%     \label{fig:motivating2}
% \end{figure} 
Consider a concrete example, where an IP user attempts to purchase a micro-controller from an IP vendor, specifically the abstracted micro-controller unit as depicted in Figure~\ref{fig:design}. The Verilog-written module \texttt{controller} provides four functional interfaces: serial data transmission ports I2C (line 15) and UART (line 17), wireless port WiFi (line 13), and a debug port (line 19). The \texttt{controller} can enable different functions through the input signal \texttt{control}. If the IP user wants to integrate wireless function of micro-controller into their product, they could use assertion-based formal verification technique to verify the wireless function. We can formalize just such an assertion as the SystemVerilog Assertion (SVA)
%
\begin{equation}\label{eq:assert}
\text{assert property: } \text{control} == 4'b0001 \, |\rightarrow \text{state} == 2'b01
\end{equation}
%
This assertion specifies that when the \texttt{control} is equal to the macro of the WiFi ({\tt 4'b0001}), the controller should always enable the wireless transmission by transitioning to \texttt{state} {\tt 2'b01}.

% shows a trading example in precision agriculture,. A simplified controller sold by microcontroller developers is commonly used in agriculture systems and provides three interfaces: 1) I2C and UART for wired data transmission, 2) WiFi for wireless data transmission, and 3) a debug mode for testing. Most agritech companies have been using the wired protocol to build a centralized tree-based network embedded system. In particular, they utilize an I2C port to link the sensor and a UART port to collect and aggregate the data. These companies, when purchasing the IP as IP users, may only focus on verifying assertions about I2C and UART. However, the wired network suffers from a single point of failure and limited scalability. Some agritech companies, therefore, might evolve their business model for services based on the wireless network. The wireless network is not only more stable and scalable but also provides an innovative alternative to conventional methods of measuring soil moisture~\cite{ding2020strobe}. These companies will switch to the assertion for WiFi functional checks in the verification phase. 
% To verify the new system, assertionis now 
% The WiFi-based mesh network\cite{wang2006wireless} is recently adopted by some agritech companies, 

% Some agritech companies decide to evolve their service by transitioning the centralized network to a WiFi-based mesh network\cite{wang2006wireless}. The Wifi module can also provide an innovative alternative to conventional methods of measuring soil moisture\cite{ding2020strobe}. %The UART port, previously utilized for data transmission, is now being substituted by the WiFi module.



% To collect moisture and temperature data, users used to utilize an I2C port to link the sensor (like SHT35\cite{Sensirion_Humidity_Sensors}) and a UART port to transmit the collected data to the upstream microcontroller (like MKE18F\cite{KE1xFP100M168SF0}) for data aggregation. 
% When they purchase IP as IP users, they only 
% Interfaces  reveals the business model that can be confidential. 

% IP design offers various APIs, such as I2C, WiFi, UART, SPI, and ADC(similar to ESP32 \cite{esp32refmanual}).
% The controller's functionality can be enabled based on the signal \lstinline[style=vcode]{control} and output register \lstinline[style=vcode]{state} provides four corresponding functions: Debug, WiFi, I2C, and UART.
% Traditionally, the Agritech company, as IP users who need to purchase the IP design from IP vendors, choose to use a wired protocol to build a centralized network embedded system. To collect moisture and temperature data, users used to utilize an I2C port to link the sensor (like SHT35\cite{Sensirion_Humidity_Sensors}) and a UART port to transmit the collected data to the upstream microcontroller (like MKE18F\cite{KE1xFP100M168SF0}) for data aggregation. 

% The assertions designed for I2C and UART are checked by the user for practical use. However, this tree-based network suffers from a single point of failure and limited scalability, Agritech decides to evolve its service by transitioning the centralized network to a WiFi-based mesh network\cite{wang2006wireless}. The Wifi module can also provide an innovative alternative to conventional methods of measuring soil moisture\cite{ding2020strobe}. %The UART port, previously utilized for data transmission, is now being substituted by the WiFi module.
% To validate the new system, assertion \lstinline[style=vcode]{assert property (control == 4'b0001 |-> state == 2'b01)} is now designed for WiFi functional checks.
% \noindent
% {\bf Bidirectional privacy.} 
% In the above scenario,
% The bidirectional privacy protocol plays an important role in this hardware trading. 
In this case, both the IP user and the IP vendor possess strong privacy concerns. The vendors wants to prevent their valuable IP design from leaking. The Verilog source code illustrated in Figure \ref{fig:design}, containing hardcoded information such as a password (Line 18), could serve as a private access point to the chip. They prefer to release the source code only after the completion of the business contract to limit any potential breach.
IP users share similar concerns when sharing assertions with IP vendors, especially when the functions being verified are closely related to their proprietary techniques. For instance, if wireless communication is the core improvement in their next-generation products, the the checking of WiFi-related assertions should not be disclosed before the product launch event. Such leaks could damage the company's reputation and allow competitors to misappropriate patented information.

% relying on I2C and UART functionalities for tree-based networks. However, their future system evolved into a mesh-based network. If the IP user shares their modified checking assertion with the IP vendor, the vendor may be able to speculate about the user's future plans--the IP user may be working on a new product that uses a wireless network topology with a new technique.
% This information could be harmful if IP vendors disclose it to the IP user's competitors.
% In other words, the IP user does not intend to include wireless capabilities in this module and plans to use the design solely for data collection and transmission. This inference could potentially expose the product's features and unintentionally reveal future product plans before the official launch.
%This module as a submodule of a large-scale system plays as a controller which accepts signal \lstinline[style=vcode]{passwd} and \lstinline[style=vcode]{control} as input. Based on the different input value, the controller will output register \lstinline[style=vcode]{state} which switch the entire system to different modes including \texttt{FUNC1},\texttt{FUNC2},\texttt{FUNC3} and \texttt{DEFAULT}. The IP user who has the functional assertion \lstinline[style=vcode]{assert property (control == 4'b0010 |-> state == 2'b10)} wants to confirm that this module work correctly in \texttt{FUNC2} mode. From the IP vendor's perspective, they do not want to expose the hardcoded password 4'b1111 as an additional backdoor for accessing the FUNC1 mode. They intend to keep this information confidential until the business contract is finalized. From the IP user's perspective, as their product only requires certain functionalities of the controller, they do not wish to disclose their future product plans. Specifically, they want to prevent the IP vendor from knowing that their product will utilize the FUNC2 mode before the product is officially launched. In this scenario. bidirectional privacy needs to be provided.
% A quick example is demonstrated to illustrate the entire privacy preservation verification process. The IP vendor, who possesses the raw RTL design (shown in Listing \ref{lst:verilogtop}) doesn't want to reveal any design detail prior to signing the business contract. Specifically, The output signal \lstinline[style=vcode]{y} in the design can be controlled by two external signals \lstinline[style=vcode]{ctrl_a} and \lstinline[style=vcode]{ctrl_b}. The IP user cannot easily determine the driver signal without inspecting the design or related document. On the other hand, The IP user who is interested in understanding the functionality of signal \lstinline[style=vcode]{ctrl_l} holds the checking assertion \lstinline[style=vcode]{assert property (ctrl_a == 1'b1 |->y == 1'b1)}
% However, the IP user doesn't want to disclose his intention, i.e., the IP user realizes that the exposure of assertion before finalizing the business agreement can lead to confidentiality breaches related to future product integration. Both parties involved in this scenario aim to safeguard their respective confidential information until the verification process is completed and the business contract is officially signed.
\begin{figure}[ht]
    \centering
\begin{lstlisting}[style=motivating, basicstyle=\ttfamily\scriptsize]
module CryptoCore (
    input  wire         clk,
    input  wire         rst_n,
    input  wire [127:0] plaintext,     // Input message
    input  wire [127:0] key,           // Encryption key
    input  wire [3:0]   sel,           // Crypto mode
    output wire [127:0] ciphertext,    // Encrypted output
    output wire [127:0] cert_hash      // Digest
);

// Internal signals
wire [127:0] internal_result;
wire [127:0] internal_cert_hash;

// Real implementation is kept confidential by the vendor.
endmodule
\end{lstlisting}
\caption{An abstracted CryptoCore that exposes I/O interfaces and a few internal signals to users while keeping implementation details confidential.}
\label{fig:design}
\end{figure}

We explain the interaction between IP users and vendors in \tool{} using the above example. The IP user starts by constructing the assertion to verify as in Equation~\ref{eq:assert}. As noted, the hardware module controller depicted in Figure \ref{fig:design} features four interfaces: WiFi, I2C, UART, and Debug. The activation of these interfaces is determined by the value of the \texttt{state} variable, which is contingent upon the input value of \texttt{control}. The IP user therefore sends the keywords \texttt{control} and \texttt{state} to the IP vendor in order to synchronize the signals of interest in the verification. This information ensures that IP vendor maintains a mapping from bitvector signals to Boolean variables for subsequent namespace synchronization, establishing the candidate signal set $\mathbb A$.


% \begin{figure}
%     \centering
%         \begin{lstlisting}[style=smtlib2,basicstyle=\ttfamily\scriptsize]
% // Define constants
% controller.WIFI <--> #b01 
% controller.I2C <--> #b10
% controller.Uart <--> #b11
% controller.Debug <--> #b00
% // Control logic
% controller.state <--> 
% (let ((a!1 (ite (= #x2 |controller.control#0|)
%  |controller._rn1_state#0|
%   (ite (= #x4 |controller.control#0|)
%    |controller._rn2_state#0|
%     (ite (= #xf |controller.passwd#0|)
%      |controller._rn3_state#0|
%       |controller._rn4_state#0|)))))
%        (ite (= #x1 |controller.control#0|) 
%         |controller._rn0_state#0| a!1))
% // State variables
% controller._rn0_state <--> #x00000001
% controller._rn1_state <--> #x00000002
% controller._rn2_state <--> #x00000003
% controller._rn3_state <--> #x00000000
% controller._rn4_state <--> #x00000003
% \end{lstlisting}
% \caption{Encode controller into SMT-LIB 2}
% \label{fig:smt}
% \end{figure}






% \sam{we should do this using ``\textbackslash ref'' so that they are all correct and linked}). 

% IP design information that matters to assertion interests. 
% Since this property can be verified within a single clock cycle, IP users also send the signal keywords \texttt{control} and \texttt{state}, along with a time-bound of \texttt{1}, to IP vendors. \ning{This does not make sense to me. What is a single clock cycle? What is the message this sentence wants to convey in this context?}
Upon receiving this signal keyword information, the IP vendor generates an SMT formula representing their IP design. The SMT formula for IP design example in Figure~\ref{fig:design} is shown in Figure~\ref{fig:smt} \sam{WHERE IS THIS?}. Meanwhile, the IP user specifies their assertion as an SMT formula. In our example, the IP user will use the formula:
$
\texttt{controller.control\#0} == 1 \land \neg (\texttt{controller.state\#0} == 1)
$
This formula represents an error where the controller can not enable WiFi functionality. 
% represents the negation of the assertion that is \lstinline[style=vcode]{(control == 4'b0010 & state != 2'b01)}. 
The \textit{UNSAT} of the conjunct of formulae from IP users and vendors asserts that the error will never be triggered. 
%

These SMT formulae are further translated to CNF. For formulae of our interests, i.e., the formulae for hardware IPs and assertions, using tactics \textit{Bit-blasting} and \textit{Tseitin transformation} will be sufficient for such translation. 
% To decide \textit{SAT/UNSAT} of the conjunct of the formulas provided by both parties, \textit{Bit-blasting} and \textit{Tseitin transformation} tactics are leveraged to translate SMT to SAT in CNF (Figure~\ref{lst:cnfdesign} and Figure~\ref{lst:cnfassertion_before}). 
% \ning{IP vendors send variable mapping back to IP users. IP users update the CNF integer identifiers (Figure~\ref{lst:cnfassertion_after}) so that the conjunct of the formulae has the same semantics and namespace.
% put to the implementation details}
% \input{img/dimacs}
% Both parties further generate CNF from SMT.
% IP users and vendors then convert their SMT formulae to CNF formulae with \textit{Bit-blasting} and \textit{Tseitin transformation}. During this conversion process, a variable mapping is recorded that correlates each signal—specifically \texttt{control} and \texttt{state}—to its corresponding variable in the CNF. \ning{add explaination why Bit-blasting and  Tseitin transformation is sufficient.}
% \ning{This paragraph is very hard to follow.}
% Then, \textit{Bit-blasting} and \textit{Tseitin transformation} tactics are further utilized to get the CNF of the design(in Appendix Listing \ref{lst:cnftop}). 
% Simultaneously, IP users encode their assertions into CNF similarly (in Appendix Listing \ref{lst:cnfsvatop_before}). To verify this assertion against the design in SAT solver\ning{what "verify XXX in SAT solver means"?}, the negated assertion \lstinline[style=vcode]{control == 4'b0010 & state != 2'b10)} is used. Once IP users receive the variable mapping, the integer identifiers in CNF are updated accordingly(in Appendix Listing \ref{lst:cnfsvatop_after}) so that both design CNF and assertion CNF can be conjoined based on the same semantics.
Finally, IP vendors and IP users jointly decide the satisfiability of the conjunction of their CNFs. 
% The CNFs should be kept private as they reflect the sensitive information of the design and the properties. Most existing SAT solvers do not protect privacy. ppSAT enables two-party SAT solving, but it is not scalable to our instances.

%The reason behind the poor performance of ppSAT is their heuristics are designed for general formaulae. On the other hand, formulae in our setting have special structures. In this paper, we propse a new \ning{XXX} for privacy preserving SAT solving, tailored for hardware verification. 

%The core of our work is 
%If \textit{UNSAT} is returned, no counterexample is provided for the negated assertion, indicating that the IP function follows the desired design intention, thereby verifying the correctness of the IP.


% \begin{lstlisting}[style=smtlib2, label={lst:smtsvatop},caption={Assertion\_SMT-LIB 2}]
% (assert
%  (let (($x124 (and (distinct |controller.state#0| (_ bv2 2)) true)))
%  (let (($x60 (= |controller.control#0| (_ bv2 4))))
%  (and $x60 $x124))))
% \end{lstlisting}



%, respectively.


==> sections/ppmc_part.tex <==
\subsection{Zero Trust Verification Framework}

A key guarantee of our procedure is that the IP user is never provided the original RTL code. Instead, the IP vendor only exposes its design in an encrypted manner through the \texttt{PPMC} interactive protocol. The properties of the IP user in CTL are also kept private by the protocol. Such a distributed verification procedure ensures protection and privacy of the IP designs and the properties, as shown in Figure \ref{fig:system}. The \texttt{PPMC} tool automatically checks the design against the properties and reports the output to both parties.

% Figure \ref{fig:system} also demonstrates the \texttt{PPMC}-based formal verification workflow. EDA Service Provider constructs the \texttt{PPMC} checking protocol, then designates ports \texttt{PPMC} party 1 and \texttt{PPMC} party 2 to IP User and IP Vendor separately. IP user translates natural language property into CTL formula and submits it to \texttt{PPMC} party 1 while IP vendor provides the design model in Kripke structure. The \texttt{PPMC} runs oblivious transfer, and the garbler collects the encrypted data and runs model checking to compute the Boolean output. Then, both sides get notified through the EDA-designated port. IP User and IP Vendor are prevented from spying on each other through garble circuit and the EDA service hides the operation pattern through the modified oblivious algorithm to make the different verification procedures indistinguishable. All three parties protect their privacy through the proposed framework.

Figure \ref{fig:system} represents the zero trust verification workflow with the three stakeholders of the IC design process. The EDA service provider coordinates the use of the \texttt{PPMC} tool. All cryptographic operations and communication are performed by Party 1 and Party 2, the IP user and IP vendor, respectively.
Initially, a data format is shared (likely by the service provider) between the IP user and the IP vendor, indicating name space information, such as signal and port names. Based on those data, the IP user develops and translates a natural language property into the CTL formula $\varphi$ and inputs it as Party 1. Meanwhile, the IP vendor abstracts the RTL code of the IP into the Kripke structure $\mathcal{M}$ (using, as we shortly describe, Algorithm~\ref{alg:kripke}) and then inputs it as Party 2. 

The two parties then execute the \texttt{PPMC} protocol to compute the Boolean value $b$ that indicates whether $\mathcal{M} \models \varphi$. At the conclusion of the protocol, $b$ is output to both the IP user and the IP vendor. Throughout the computation, the underlying secure computation primitives (symmetric key encryption, garbled circuits, and oblivious transfer) prevent the IP user and IP vendor from learning anything about the other party's inputs, and also prevent the EDA service provider from eavesdropping if they are used as a communication proxy.
% The EDA service hides the operation pattern through the modified oblivious algorithm to make the different verification procedures indistinguishable. All three parties protect their privacy through the proposed framework.




% The \texttt{PPMC} framework is compiled to binary file and distributed to both IP vendor and IP integrator sides. Two party prepare CTL $\varphi$ and Model $M$ to set up the \texttt{PPMC} protocol. Through oblivious transfer, the garbler collects the encrypted data and runs model checking to compute the Boolean output. Then, both sides get notified for the checking result. Since the model checking algorithm is modified to be data oblivious, the memory access pattern won't reveal any sensitive information throughout computation. Therefore, The properties get verified under privacy preserving mode without revealing any information to both sides.





% The task of converting the properties of the IP user in natural language to formal properties can be carried out by a \textit{specification engineer}, who may be an in-house security team, or a trusted third party of the IP integrator. Apart from developing formal properties, the specification engineer can also run test on the $\textsf{\texttt{PPMC}}$. 

%\textcolor{blue}{The example needs revision. We have to talk about a security property and a Verilog model that are obfuscated. Otherwise, it will be a regular hardware model checking problem. Reduce the number of references to make space. Example of obfuscated RTL code: https://www.aldec.com/en/support/resources/documentation/articles/1586}

The task of converting properties of interest from natural language to formal language (CTL) is carried out by the IP user. An example of how CTL can be used to specify a simple property is the Common Weakness Enumeration (CWE) 1271~\cite{CWE1271}. This CWE is a \textit{reset property}, stating that `all registers holding security-critical information should be set to a specific value on reset' (but is not necessarily reached on every run).
Expressed in CTL, this can be written as 
$$\varphi \equiv \text{AG}(\texttt{reset} \rightarrow \text{X} (\neg \texttt{lock\_jtag})).$$
where, AG means \textbf{a}lways \textbf{g}lobally (and using our minimal CTL grammar, can be rewritten as $\text{AG } \varphi \equiv \lnot(\text{E } [\top \text{ U } \lnot\varphi])$).
In PSL, this is expressed as:
%
$$\texttt{always (true[*]; reset) |=> (!lock\_jtag)}.$$
%
In natural language, this can be interpreted as `for all execution traces, after a reset, the security critical $\texttt{lock\_jtag}$ value must be 0'. This weakness is demonstrated in the Verilog code shown as code in Listing 1 of CWE 1271~\cite{CWE1271}. Here, \texttt{lock\_jtag} is a flip-flop triggered by a positive clock edge that is used to manage access to the debug interface. The issue is that the state of the \texttt{lock\_jtag} flip-flop will be in an unknown state after the circuit is reset. An attacker could reset the circuit many times until the bit grants access to the debug interface. To avoid this, line 2 can be uncommented -- in which case the code will satisfy the CTL property stated above.

%\noindent\begin{minipage}{.24\textwidth}
\begin{lstlisting}[
style=flang,
label=lst:secv,
numbers=left, 
xleftmargin=\parindent, 
%basicstyle=\footnotesize\ttfamily, 
caption=CWE-1271]
  always @(posedge clk) begin
    //if (~reset) lock_jtag <= 0;
    if (en) lock_jtag <= d;
  end
\end{lstlisting}

%\vspace{-.1in}
%\end{minipage}\hfill
%\begin{minipage}{.22\textwidth}
% \begin{lstlisting}[style=flang,label=lst:q, %basicstyle=\footnotesize\ttfamily,
% caption=Obfuscated RTL]
% always @(posedge s_62f9fbcc145dd2fd44) 
% begin
% if (s_31426f27facd30c) 
% s_aa0c845157396d9867<= s_0c9aded5f2fe3;
% end
% \end{lstlisting}
%\vspace{-.1in}
%\end{minipage}

\subsection{Modeling Algorithm}\label{sec:algorithm}

\begin{figure}
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \resizebox{\columnwidth}{!}{\input{figs/fsm}}
        \caption{Original FSM of \texttt{b02}}
    \end{subfigure}%
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \resizebox{0.8\columnwidth}{!}{\input{figs/kripke}}
        \caption{Kripke structure of \texttt{b02}}
    \end{subfigure}
    
    \caption{An FSM and corresponding Kripke structure for benchmark \texttt{b02} from Table I. Once we extract the FSM from the RTL code, Algorithm~\ref{alg:kripke} visits each state and builds the digraph based on the relevant atomic propositions. In this example, our property is related to a 1-bit signal \texttt{U}.}
    \label{fig:fsm}
    %\vspace{-0.1cm}
\end{figure}

As CTL properties cannot be directly checked against the RTL code, we first require the IP vendor to transform the hardware design $M$ into a Kripke structure $\mathcal{M}$. As described in Sect.~\ref{sec:pre-kripke}, a Kripke structure is a digraph whose edges represent state transitions and whose nodes are labeled with system states. To obtain a Kripke structure from the RTL code, we first extract the design's Finite State Machine (FSM), using the approach of~\cite{orlando2022fsm}. This gives us the state transitions. We then convert this FSM to a Kripke structure by adding labels to the nodes.

In Algorithm~\ref{alg:kripke}, we illustrate how we convert an FSM from RTL code into a Kripke structure. Algorithm~\ref{alg:kripke} accepts the HDL's Abstract Syntax Tree (AST) as input and produces a Kripke structure as output. After identifying the initial FSM state $s'_0$ and the state transition function $\delta$, the AST is traversed to identify the property-related signals that form the set of atomic propositions, $ap_{i}$ for $i \geq 0$. A labeling function in a Kripke structure maps each state/node to a set of corresponding properties/signals. Therefore, the tuple, $s_0 = (s'_0, ap_0)$ where, $L(s'_0) = ap_0$ can be used to represent the initial state of the Kripke structure. Based on the FSM's state-transition function $\delta$, a new reachable FSM state $s'_i$ is visited, and the new state $s_i = (s'_i, ap_i)$ is added to the existing digraph. The complete Kripke structure is built after iterating all reachable states and their corresponding properties/signals.

Figure \ref{fig:fsm} shows an example of an FSM and its corresponding Kripke structure. The FSM encodes the IP: \texttt{b02} from Table \ref{tab:exp}. The property we investigate only includes a single signal \texttt{U}, which is a 1-bit signal. Thus, Algorithm~\ref{alg:kripke} looks up the AST and searches for the assign statement of \texttt{U} in order to collect the atomic propositions. The constructed tuple $(s'_i,ap_i)$ represents a state $s \in S \subseteq S' \times 2^{AP}$ for $S'$ the set of states of the FSM.
\begin{algorithm}
\begin{algorithmic}[1]
    \Function{FSMtoKripke}{$ast$}
        \State {$s'_{0},\delta \gets get\_fsm(ast)$}
        \State{$ap_{0} \gets get\_atomic\_proposition(ast,s'_{0})$}
        \State {$init\_state \gets s_0 = (s'_{0},ap_{0})$}
        \State {$visited \gets init\_state$} 
        \State{$push(queue, init\_state)$}
        \State{$ digraph \gets \varnothing$}
        \While{$ queue \neq \varnothing$}
            \State{$pop(queue, state)$}

            \For{$s'_i \in get\_next\_states(\delta,state)$}
            \State{$ ap_{i} \gets get\_atomic\_proposition(ast,s'_{i})$}
            \State{$new\_state \gets s_{i} = (s'_i,ap_i)$}
            \State{$update\_graph(digraph,state,new\_state)$}
            \If{$new\_state \notin visited$}

            \State {$queue \gets queue \cup \{new\_state\}$}
             \State{$visited \gets visited \cup \{new\_state\}$}
            \EndIf

            \EndFor
        \EndWhile
        \State \textbf{return} {$digraph$}
    \EndFunction
\end{algorithmic}
\caption{Convert FSM to Kripke Structure}
\label{alg:kripke}
\end{algorithm}
%
% \vspace{-0.4cm}

\subsection{Privacy Preserving Model Checking}

We refer the reader to~\cite{judson2020privacy} for a detailed description of the $\texttt{PPMC}$ protocol. At a high level, the protocol works by having the IP vendor generate an AES-128 secret key $k$, encrypt information about the transition and label matrices of $\mathcal{M}$, and then send the resultant ciphertexts to the IP user. The parties then execute $m = |\varphi|$ rounds of a secure computation protocol. In each round, they interactively compute a model checking procedure for each of the five operators in the reduced CTL grammar. The output of these subprotocols are themselves AES-128 ciphertexts, encrypted by $k$ through executions of the AES-128 encryption algorithm `in-circuit'. The IP user then chooses whichever ciphertexts correspond to the right operator in $\varphi$ to carry over to the next round of the protocol. 

The subprotocols work by implementing various oblivious graph algorithms as garbled circuits (themselves based on symmetric key encryption and oblivious transfer)~\cite{4568207}, with the IP vendor as garbler and the IP user as evaluator. The protocol runs in time $O(mn^2)$ for $n = |\mathcal{M}|$, and so requires no asymptotic overhead, though the oblivious nature of the algorithm means it \textit{always} takes that long, and there is meaningful concrete overhead from the cryptographic operations (especially the `in-circuit' AES executions). As the five operators are independently checked, the protocol is amenable to parallelization within each round.

==> sections/protocol.tex <==

\begin{tikzpicture}
\usetikzlibrary{calc,arrows,matrix,positioning,chains,shapes,automata}
	\matrix (m) [
			matrix of nodes,
			column sep=0.5cm,
			row sep=0.8cm,
			nodes={
				draw=none,
				anchor=center,
				text depth=0pt,
				text width=3.75cm,
				text centered,
			},
		] {
    IP User	    &		& IP Vendor	\\[-7mm]
$\spec \from \text{Specification}$%
                &		& $\design \from \text{ Design}$%
                                    \\[-8mm]
$\tb \from \text{Time Bound}$%
                &		& 
								\\[-8mm]
$\signalset =\textit{parse}_{spec}(\spec,\tb)$%
                &		&
								\\[-8mm]
			& $\signalset$, $\tb$%
					&			\\[-6mm]
$ \speccnf,\maps =\textit{parse}_{sat}(\spec,\tb)$		&		& $\pdesign =\textit{prune}(\design,\signalset)$%
                                    \\[-8mm]
                &		& $\heuset = \textit{extract}(\pdesign)$%
                                    \\[-8mm]
                &		& $\designsmt=\textit{translate}(\pdesign)$%
                                    \\[-8mm]
                &		& $\designsmt^{\tb}=\textit{unroll}(\designsmt,\tb)$%
                                    \\[-8mm]
                &		& $\designcnf,\mapd,\heulitset =\textit{parse}_{sat}(\designsmt^{\tb},\heuset)$%
                                    \\[-6mm]               
			& $\mapd , |\designcnf|_v,|\designcnf|_c$%
					&			\\[-6mm]
$\speccnf' = \textit{update}(\maps,||\speccnf||,\mapd)$%
			&		& 
								\\[-4mm]
			& $\texttt{hw-ppsat}(\speccnf' \wedge \designcnf,\heulitset)$%
					&			\\[-6mm]
			% & $b \in \{0,1\}$		
   %                      &
   %                                  \\[-6mm]
	};

	\draw (m-1-1.south west)--(m-1-3.south east);
        \draw [latex'-latex'](m-13-2.south west) -- (m-13-2.south east);
        % \draw [latex'-latex'](m-14-2.south west) -- (m-14-2.south east);
	\def\arrowdata{
		5/2/west/east,
		  11/2/east/west%
		% 8/2/east/west,
		% 10/2/west/east%
	}

	\foreach \x\y\src\dst in \arrowdata {
		\draw[-latex'] (m-\x-\y.south \src) -- (m-\x-\y.south \dst);
	}

\end{tikzpicture}

==> sections/rebuttal.tex <==
\newpage

\begin{center}  
\textbf{\Large Response Letter}
\end{center}

We thank the reviewer for the constructive comments. We took all the comments seriously and made our best efforts to improve the manuscript. Below please find our responses to the reviewers’ comments.

\vspace{.1cm}
\noindent\textbf{Reviewer 1: Reject--No familiarity}

\begin{quote}
The paper is poorly written, formalises none of the hypotheses it makes not states any formal result. It does not give any formal statement about the soundness of the verification. It also lacks any statement about what information remains protected.
\end{quote}
\textcolor{red}{
% Our framework utilizes a well-established secure multiparty computation method. We don't need formal statements as we cite the related work. We further extend the secure multiparty computation theory into the hardware formal verification domain with a hardware-oriented heuristic. The result shows that our framework could accelerate the verification process compared with existing state-of-the-art methods.
We have refined the language of the paper to ensure that it clearly presents our method. However, since our framework utilizes a well-established secure multiparty computation method, the formal statements can be found in the citations in the related work section. We further extend secure multiparty computation theory into the hardware formal verification domain with a hardware-oriented heuristic. The results show that our framework can accelerate the verification process compared to existing state-of-the-art methods.
}

\begin{quote}
The approach relies on a middle organisation, but does not discuss the trust in that organisation. it seems the requirement for both users and vendors to send their design to another entity may raise exactly the same issue as the paper was trying to address in the beginning.
\end{quote}

\textcolor{red}{
% We don't rely on any middleman. Our framework only requires the CNF input from IP users and IP vendors. The formal checking procedure is performed using the extended ppSAT. The generation of CNF from RTL is performed locally. Based on our semi-honest threat model. Both parties are responsible for the correctness of the generated CNF.
BlindMarket operates without the need for a middle organization, as all procedures are automated using the developed tools. Specifically, the proposed framework requires only the CNF input from IP users and IP vendors. The formal checking procedure is conducted using the extended ppSAT tool. The CNF is generated locally from RTL using the developed parser. Based on the proposed semi-honest threat model, both parties are responsible for ensuring the correctness of the generated CNF.
}

\begin{quote}
Not only the paper lacks formal guarantees, but it also makes several statements that seem to imply the method has limitation that are not discussed. Section IV.E mentions heuristics but does not make it clear whether the use of heuristics may mean verification may fail / may not preserve all information. Also, IV.F mentions unavoidable disclosure but does not discuss it. 
\end{quote}
\textcolor{red}{
The objective of heuristics is to accelerate the solving process by reordering the search path without affecting the correctness of the verification result. The unavoidable disclosure is the control signal set, which we discuss as a trade-off between time and privacy. This optimization enables BlindMarket to achieve significant efficiency improvements. The corresponding clarifications have been added to the resubmitted version.
}

\begin{quote}
The experiments are not very well discussed either, and it is unclear what the conclusion would be in terms of scalability, information protection, etc.
\end{quote}
\textcolor{red}{
% We formally verify our proposed framework in a real-world example for privacy-preserving hardware verification. First of all, we show that our framework could be used in IP-level hardware functional verification. Second, we compare our optimization, and shows a great improvement compared with the state-of-the-art work.
The experimental section formally validated BlindMarket using a real-world example for privacy-preserving hardware verification. The results show that the proposed framework is effective in IP-level hardware functional verification. Additionally, the comparison results demonstrate significant improvements over state-of-the-art methods.
}
\begin{quote}
P1: widely adapted AMD... $->$ by

P2: four interfaces: ... then lists 3 points
\end{quote}
\textcolor{red}{
We have corrected the typo in the revised version.
}

\vspace{.1cm}
\noindent\textbf{Reviewer 2: Weak reject--No familiarity}

\begin{quote}
The examples are hard to follow. For example, Figures 2 and 3 are not explained and the properties that are verified are also not clear to me. There is no explanation for why we want these properties to hold. 
\end{quote}
TODO

\begin{quote}
Similarly, Figure 4 shows IP designs in CNF (DIMACS) form without any explanation of what those numbers mean and this trend continues
for the other figures as well.   
\end{quote}
\textcolor{red}{We deleted Figure 4 as well as checked the other figures to make sure each one has a corresponding explanation.}


\begin{quote}
There are numerous grammar errors and acronyms as well as other names (e.g. Subsetting, candidate signal set, giant step, ROM) which are not explained.  
\end{quote}
\textcolor{red}{
We corrected the typo and added the following explanation.\\
We added the explanation of Subsetting in Section \ref{subsec:prune}:\\
Design subsetting is an optimization technique when the analysis focuses on a specific component or aspects of a system. In the hardware domain, RTL subsetting is particularly beneficial for resource-intensive analysis like formal verification as the irrelevant state variables and transition function are excluded in data encoding.\\
We added the explanation of the candidate signal set in Section \ref{subsec:assertion}:\\
\tool parses in the specifications provided by IP users and translates the assertion into the bit vector logic formula. The candidate signal set $\mathbb A$ collects all assertion-related signal variable names.\\
We clarify the acronym of ROM in Section \ref{subsub:2darray}:\\
Read-Only Memory (ROM).\\
We added the explanation of giant step in Section \ref{subsec:ppsat}:\\
The \texttt{ppSAT} protocol~\cite{luo2022ppsat} provides a tailored solution to a two-party SAT-solving problem. The construction works by taking the classic DPLL decision procedure for Boolean propositional logic~\cite{davis1960computing, davis1962machine} and lifting it into a secure protocol through a data-oblivious reformulation of the core reasoning loop, including support for multiple decision heuristics. This data-oblivious DPLL consists of a sequence of giant steps and each giant step sequentially executes oblivious variants of the five core small-step algorithms including UNITSEARCH, DECISION, CHECK, BACKTRACK, and PROPAGATION. This algorithm is then deployed into a secure computation environment by using standard garbled circuit designs and tooling.
}
\begin{quote}
Furthermore, a section describing the security/privacy guarantees of their BlindMarket protocol is missing. What are the guarantees the protocol gives?   
\end{quote}
\textcolor{red}{
TODO
}

\begin{quote}
Multiple acronyms (IP, EDA) used in the abstract are not defined there, while others are (3PIP, CNF, etc.)
\end{quote}
\textcolor{red}{
We clarify the acronym of EDA, 3PIP in the Introduction:
Third-party (3P).\\
Intellectual Property (IP).\\
Electronic Design Automation (EDA).\\
Conjunction Normal Form (CNF).\\
}

\begin{quote}
The sentence "formal verification is completeness and uses mathematical methods to or disprove the correctness of the design". What does this mean?  
\end{quote}
\textcolor{red}{
We want to claim formal logic-based verification is better than simulation and emulation for IP verification. We revised it and added more explanation in the introduction:\\
Formal logic-based verification is used as the basic technique in our framework. Existing simulation (and emulation) based privacy-preserving IP verification methods\cite {hashemi2022garbled,mouris2023mploc} require extensive test suites to cover and verify the correctness of the design functionalities. Formal verification in contrast provides a rigorous approach to examine all possible hardware states without the need for test input.
}

\begin{quote}
In the contributions, it is listed that a SAT solver is used. However, in the preliminaries, the authors only talk about SMT solvers. Similarly, it is not clear to me (from
the text) if the ppSAT protocol can be used for SMT solvers as well.
\end{quote}
\textcolor{red}{
We use SAT solver \texttt{hw-ppSAT} in our framework. However, before the generation of CNF, we first parse the design into SMT LIB 2 with optimization, which then be converted into CNF.\\
We revised the Section \ref{subsec:overview} as follows:\\
The design in SMT-LIB 2 is further unrolled into CNF with a bound of $b$ using \textit{Bit-blasting} and \textit{Tseitin transformation}.
The RTL design in CNF and control signal set $\mathbb C$ is the final input to (\texttt{hw-ppSAT}) from IP vendors' side.
With the provided design CNF, property CNF, and heuristic input, SAT solver (\texttt{hw-ppSAT}) conducts a two-party computation to accomplish the design verification.
}
\textcolor{red}{
We revised Section \ref{subsec:overview} to clarify our framework and the use of SAT solver and SMT solver.
}

\begin{quote}
It is unclear to me how natural language can be used as assertion language. Can the authors give examples of how this looks like and how it is parsed?  
\end{quote}
\textcolor{red}{
We could define the functional property in nature language, which could be further translated into Systemverilog Assertion (SVA) or Property Specification Language (PSL) to verify the hardware design. The translation from Natural language to PSL/SVA is manual, we detail the process in Section \ref{subsec:assertion}. We also walk through it in the motivating example.
}

The intro in VI mentions that the framework is introduced in Section IV, which already happened.
The motivating example in III feels too specialized and diverts the reader from the goal.
The assertions provided are very small. The authors say they want to verify functional correctness. What if the assertion queries are getting bigger? Do the authors have
results for this case as well?   




\vspace{.1cm}
\noindent\textbf{Reviewer 3: Accept with shepherding--Some familiarity}

- The experiments require long times to run even on small test cases, meaning that the approach likely doesn't scale to real-world scenarios
- The experiments show just a small number of single-assertion queries, which only allows the user to determine a few properties of the IP (compared to say, long series of simulations)


The paper's presentation starts with introduction, background, and a motivating example.  This is all fine, but there's extra space available, and it's conventional to have an adversary model somewhere in the first few pages.  This could help make the paper's security claims more precise.  As it stands, the paper comes across as a presentation of a framework and experimental results without much rigor in the security analysis.

The paper isn't convincing in motivating why it's important to protect the user from the vendor.  For example, page 1 says: "On the other hand, IP vendors might collect functional requirements from IP users and examine the assertions. ... Attackers could engage in reverse engineering to mount highly targeted system-level cyberattacks."  What's the attack here?  Is that the IP vendor accidentally leaks the user's IP requirements to the public, and an outside attacker uses the leaks for reverse engineering?  Is the vendor mounting cyberattacks (which seems unlikely).  Or is the attacker an insider associated with the vendor?

\begin{quote}
page 2: argitech
page 4: " is shown in Figure 3)." mismatched parenthesis
page 4: fig 4 caption: "againstt"
Figure 4 is incomprehensible -- are readers supposed to read all these numbers?
page 4: "upon receiving A and b. BlindMarket subsets"  extra "."?  
\end{quote}
\textcolor{red}{We corrected the typo and revised the motivation example.}

\begin{quote}
 Section VI: "Table III lists the summary of the existing work and its limitations. We formally introduce our framework in section IV."  Should this say "We formally introduced" to refer back to section IV?
\end{quote}

==> sections/revision.tex <==
\section*{Responses to Reviewer Comments}

\noindent{\textbf{Response to all reviewers and track chairs:}}

\answer{\noindent We sincerely thank the reviewers for their thoughtful and constructive comments, as well as the program chairs for their time and effort in managing our manuscript. We have carefully considered all feedback and revised the manuscript accordingly to address the concerns raised.}

\answer{In the following, we first provide point-by-point responses to each reviewer's comment. For clarity, the original comments are shown in regular black text, while our responses are presented in blue. Any newly added or revised text is highlighted in italicized blue with quotation marks. The corresponding modifications in the revised manuscript are also shown in italicized blue.}

\answer{In addition, as the major revision notification includes updated requirements, we have carefully reviewed those points to ensure that no requested revisions are overlooked. Following the responses to the reviewers’ comments, we also provide a dedicated section addressing the updated major revision requirements, along with corresponding manuscript revisions presented in the same format as described above.}

\answer{Specifically, we provide detailed responses to the comments from the four reviewers in Sections A--D, respectively. In Section E, we address the ``Requirements for Major Review,'' which consist of questions selected and summarized from the reviewers' original comments.}



\subsection{Response to Reviewer 1:}
\noindent\textbf{Q1.1:} The paper does not include quantitative metrics for verification time, memory usage, or cryptographic overhead for larger, industrial-scale designs or for IP portfolios containing hundreds of cores. Given that SAT-based verification and secure 2PC are known to be computationally intensive, a deeper evaluation on larger-scale SoCs would strengthen the claims of practicality and end-to-end usability.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for this suggestion. In the following response, we first discuss the limitations of scaling \tool to large designs and then provide a quantitative analysis of the overhead as a reference for large-scale deployments.}

\answer{\input{revision/scalability}}

\answer{Additionally, we extend our evaluation in Section~\ref{subsec:overhead} to quantify the communication overhead of both 2PC and OT. Overall, both OT and 2PC overhead scale approximately linearly with the design size, but design pruning and control-flow-guided heuristics significantly reduce the effective circuit size and number of giant steps, making privacy-preserving verification practical.}


\revise{
\input{revision/Crypto_overhead}}


\vspace{.1in}\noindent\textbf{Q1.2:} The paper would benefit from a discussion of how these performance improvements translate to real-world deployment scenarios, including potential trade-offs between verification speed, IP confidentiality, and solver completeness.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for this insightful suggestion. In this response, we first discuss the trade-off between efficiency and confidentiality. We then revise the manuscript to illustrate the proposed mitigation.}

\answer{\input{revision/trade_off}}

\vspace{.1in}\noindent\textbf{Q1.3:} The framework’s complexity raises potential usability and integration concerns. BlindMarket involves multiple sophisticated steps, including CNF encoding, masking, oblivious transfer, 2PC-based verification, and ledger integration. Each step requires precise alignment between IP vendors and users, and the paper does not discuss the potential challenges of integrating these steps with standard EDA toolchains or existing verification workflows.

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this concern. In this response, we first discuss the integration of \tool into existing verification workflows, and then revise the manuscript to clarify the precise alignment required between the two parties.}

\answer{\tool is designed to operate as a lightweight preprocessing and verification layer on top of existing verification flows rather than replacing them. In practice, hardware designs written in synthesizable RTL are first processed by any static-analysis frontend that can perform dataflow analysis. The design is then translated into an SMT representation and subsequently converted into CNF following the standard SAT-based hardware verification pipeline. \texttt{hw-ppSAT} serves as the checker that enables privacy-preserving formal verification. Although current commercial formal verification tools do not natively support such capabilities, the proposed framework can be integrated as an additional execution engine for existing verification tools such as VC Formal~\cite{synopsys:vcug} or JasperGold~\cite{JasperGold}.}

\answer{We also revised the Section~\ref{sec:con} to declare the alignment required between the two
parties. As shown below.}

\revise{A practical challenge of \tool lies in its interactive protocol, where stages such as oblivious design selection and secure SAT solving require synchronized message exchanges between the IP vendor and the IP user, introducing additional latency compared with offline verification. Despite this overhead, the framework remains compatible with existing post-licensing IP protection solutions and can be integrated into current hardware supply-chain ecosystems.}


\vspace{.1in}\noindent\textbf{Q1.4:} Finally, some technical details could benefit from additional clarification. For instance, the derivation and transmission of the control-flow-guided partial-order set in hw-ppSAT is a critical optimization; more discussion of how this avoids information leakage while remaining practical would be valuable. 

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for this helpful suggestion. In this response, we first formally illustrate the transmission of the control-flow-guided partial-order set in Section~\ref{subsub:hwppsat}, which has been added to the manuscript. We then conduct extensive experiments to show that this optimization incurs negligible overhead in practice.}

\answer{The control-flow-guided partial-order set is derived locally on the vendor side. Its transmission is protected by the OT protocol following the same mechanism described in Section~\ref{subsec:ot_selection}. We further provide the detailed revised script below.}

\answer{We further quantify the overhead of the OT-based heuristic retrieval in Figure~\ref{fig:heuristic_count}.
Among all benchmarks, \texttt{adbg} has the largest heuristic set, containing 308 literals. 
Even with a 128-bit encoding per literal, the total communication cost is approximately 4.8~KB, therefore the communication overhead introduced by retrieving $\heuset$ via OT is negligible compared to the design selection and verification phases in Section~\ref{subsec:overhead}.} 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/heuristic_literal_counts.pdf}
    \caption*{Fig.~\ref{fig:heuristic_count}: \answer{Number of literals in the control-flow-guided heuristic set ($\heuset$) for each benchmark design. Even for the largest design (\texttt{adbg}), the heuristic set contains only 308 literals, resulting in negligible communication overhead when retrieved via OT.}}
\end{figure}

\revise{Unlike \texttt{ppSAT.Solve}, \texttt{hw-ppSAT} requires the IP user to provide a partial-order set $\heuset$ as an additional input, which is generated on the IP vendor side.}

\revise{To prevent information leakage, the heuristic set associated with each IP design is retrieved through the same Oblivious Design Selection protocol described in Section~\ref{subsec:ot_selection}. Concretely, the IP vendor generates a heuristic set $\heuset^k$ for each design $\phi_k$ during preprocessing and includes it in the message vector used in the OT protocol. The IP user then retrieves the corresponding heuristic set using a 1-out-of-$N$ OT via
$$
(\heuset^i, \bot) \leftarrow {\sf OT}(i, \{\heuset^1, \heuset^2, \ldots, \heuset^N\}).
$$
By the security guarantee of OT, the user learns only $\heuset^i$ and obtains no information about $\{\heuset^j\}_{j\ne i}$, while the vendor learns nothing about the user's selection $i$. Furthermore, since $\heuset$ only specifies a partial ordering of variables for branching decisions, it does not reveal structural information about the underlying circuit.}





\vspace{.1in}\noindent\textbf{Q1.5:} Additionally, it would be helpful to quantify the impact of design pruning and heuristic prioritization on solver efficiency for various classes of properties and designs.

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for this suggestion. In this response, we first discuss the impact of design pruning and heuristic prioritization on various instances. We then revise the manuscript to clarify these findings.}

\answer{The effectiveness of design pruning largely depends on the structural characteristics of the design and the locality of the verification property. Prior studies in SAT-based model checking have shown that Cone-of-Influence (COI) reduction is particularly effective for control-dominated designs, where the property depends on a relatively small subset of control signals, while the reduction is limited for datapath-intensive circuits where dependencies quickly propagate through the design~\cite{mcmillan2002applying,clarke1997model}. In Section~\ref{subsec:performance}, our experimental results further confirm this observation.}

\answer{Heuristic prioritization improves solver efficiency by guiding the search process. The work~~\cite{chen2018control} shows that control-flow information can reduce redundant exploration during solving. Our control-flow-guided heuristic follows the same intuition by prioritizing control-related variables during SAT solving.}

\answer{We further revise the manuscript to clarify this observation and include additional discussion.}


\revise{\input{revision/COI}}

\revise{Prior work has shown that incorporating structural information into variable ordering can substantially improve solving efficiency in SMT solving~\cite{chen2018control}.}



\subsection{Response to Reviewer 2:}

\noindent\textbf{Q2.1:} Include a better security statement: what each party can learn etc., and under which assumptions each privacy property hold. Broader discussion of threat model: what fails due to malicious behavior (abort, bad inputs, selective fail), and whether we can maintain a variant that is secure in the malicious setting.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for pointing out the ambiguity. We have revised the threat model to clarify that “zero-trust” refers to eliminating trusted third parties rather than implying malicious security. We also specify what each party learns under the semi-honest assumption. The revised text in Section~\ref{sec:threat} is shown below.}

\revise{\input{revision/threatmodel}}


\vspace{.1in}\noindent\textbf{Q2.2:} Clarification of mask freshness and repeated-run behavior; security argument under multiple purchases/collusion, or the protocol should be modified to not leak correlations.

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this important concern. In this response, we revise the manuscript to emphasize the necessity of mask freshness and quantify the potential attack surface when multiple purchases occur.}


\answer{We provide a formal analysis below to clarify the mask freshness.}
\answer{\input{revision/mask_freshness}}

\answer{\input{revision/assertion_signal}}
\answer{We revised Section~\ref{subsec:ot_selection} as follows:}

\revise{We require the masking matrices $({R}_P, {R}_N)$ to be refreshed for every verification session. Otherwise, colluding users could XOR masked instances obtained from different runs to cancel the masks and infer structural relationships between protected designs.}

\answer{We also enforce that the semantic map should expose a small subset of the design variables in Section~\ref{subsec:preprocess}.}

\revise{which correspond to a small subset of design variables. The semantic map assigns each observable signal a unique literal.}




\vspace{.1in}\noindent\textbf{Q2.3:} Narrow the copyright request down: either define enforceable non-transfer, or go to traceability/provenance.


\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for the suggestion. Our framework focuses on
traceability rather than enforcing strict non-transferability. We revised the Section~\ref{subsec:ip-traceability} as the reviewer suggested as follows.}

\revise{\input{revision/redistribution}}


\vspace{.1in}\noindent\textbf{Q2.4:} Augment evaluation: even a single larger or more realistic IP module and have better baselines (non-private SAT vs ppSAT vs hw-ppSAT) to show how much privacy does our construction incur.


\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for this suggestion. In the following response, we first discuss the limitations of scaling \tool to large designs and then provide a quantitative comparison with non-private SAT.}

\answer{\input{revision/scalability}}

\answer{We acknowledge that privacy-preserving verification introduces a noticeable slowdown compared with the non-private baseline. Nevertheless, since verification is typically a one-time procedure before the IP transaction is finalized, the additional overhead remains acceptable in practice. We extend our evaluation in Section~\ref{subsec:nonprivate} as follows.}

\revise{\input{revision/non_ppsat}}


\vspace{.1in}\noindent\textbf{Q2.5:} Please correct the format of reference [8] in the paper.

\noindent \textcolor{blue}{\textbf{Response:}We thank the reviewer for pointing this out. The format of reference~\cite{reuters_asml_iptheft_2024} has been corrected in the revised manuscript.}

\subsection{Response to Reviewer 3:}

\noindent\textbf{Q3.1:} Clarify the references to zero-trust and the semi-honest assumptions in the verification phase. The paper can adopt a consistent malicious model or refine the terminology.

\noindent \textcolor{blue}{\textbf{Response:}We thank the reviewer for pointing out the ambiguity. We have revised the threat model to clarify that “zero-trust” refers to eliminating trusted third parties rather than implying malicious security. We also specify what each party learns under the semi-honest assumption. The revised text in Section~\ref{sec:threat} is shown below.}

\revise{\input{revision/threatmodel}}

\vspace{.1in}\noindent\textbf{Q3.2:} Elaborate on the limitations of the traceability feature and concerns of redistribution; perhaps a watermarking mechanism to bind the IP to the certificate would be helpful.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for the suggestion. We have clarified the redistribution limitations of our framework and the potential mitigation mechanisms in Section~\ref{subsec:ip-traceability}. The revision is shown below.}

\revise{\input{revision/redistribution}}

\vspace{.1in}\noindent\textbf{Q3.3:} Discuss the risk of the Design Pruning side-channel leakage and the specific cost/efficacy of the decoy strategy.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for the comment.}
\answer{We provide a more detailed response here.} 
\answer{\input{revision/decoy_strategy}}

\answer{An additional explanation has been added in Section~\ref{subsec:ip-traceability} as shown below.}

\revise{Moreover, pruning is performed offline on the vendor side based on the user-provided property signal. Although the semantics of the property remain private to the user, the signal itself must be revealed to the vendor for COI analysis. To mitigate this disclosure, users may first submit pruning requests for multiple candidate designs as decoys to hide the actual verification target and then proceed with verification for the selected design.}

\vspace{.1in}\noindent\textbf{Q3.4:} Provide data on the communication overhead for the OT and 2PC protocols.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for this helpful suggestion. We extend our evaluation in Section~\ref{subsec:overhead} to quantify the communication overhead of both 2PC and OT. Overall, both OT and 2PC overhead scale approximately linearly with the design size, but design pruning and control-flow-guided heuristics significantly reduce the effective circuit size and number of giant steps, making privacy-preserving verification practical.}



\revise{
\input{revision/Crypto_overhead}}

\vspace{.1in}\noindent\textbf{Q3.5:} Discuss the performance of hw-ppSAT on flattened gate-level netlists in case high-level hierarchy is not available.

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this important question.}

\answer{\input{revision/flatten_netlist}}

\answer{We revised the discussion in Section~\ref{subsec:preprocess} as follows.}

\revise{Existing translation tools built on hardware synthesis frameworks typically bind the design to a specific cell library and flatten it into gate-level netlists. 
Such flattening often removes high-level semantic structures, making it difficult to express verification properties that are naturally defined at the behavioral level. 
Moreover, complex operators (e.g., multiplexers) are decomposed into primitive logic gates, which introduces a large number of auxiliary variables and clauses during CNF generation. 
Since \tool encodes the CNF as a pair of binary matrices $(P, N) \in \{0,1\}^{n \times m}$, larger values of $n$ and $m$ directly increase the computational and communication overhead of the subsequent secure protocols.}

\subsection{Response to Reviewer 4:}
\noindent\textbf{Q4.1:} The paper’s strongest claims (zero-trust trading with verifiability/confidentiality) are made in a setting where verification assumes semi-honest behavior.

\noindent \textcolor{blue}{\textbf{Response:}We thank the reviewer for pointing out the ambiguity. We have revised the threat model to clarify that “zero-trust” refers to eliminating trusted third parties rather than implying malicious security. We also specify what each party learns under the semi-honest assumption. The revised text in Section~\ref{sec:threat} is shown below.}

\revise{\input{revision/threatmodel}}





\vspace{.1in}\noindent\textbf{Q4.2:} Several benchmarks remain very costly or time out even with optimizations, raising concerns about feasibility on larger IP blocks.

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for pointing out this concern. As shown in Table~\ref{tab:exp}, by combining design pruning with control-flow-guided heuristics, 13/13 benchmarks can be verified within a reasonable time, considering that verification is typically a one-time procedure in this setting.}

\answer{\input{revision/scalability}}

\vspace{.1in}\noindent\textbf{Q4.3:} Even if transcripts are hidden, repeated SAT/UNSAT answers can enable property probing that gradually reveals design behavior; the work lacks a formal leakage discussion or query-limiting mechanisms. The design remains hidden, but the buyer learns SAT/UNSAT outcomes of style checks. Over many queries, it becomes a powerful oracle for inferring design behavior (and potentially reconstructing parts of the logic). The paper doesn’t provide a leakage model, rate limits, query auditing, or any bounds on cumulative information release.

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this important concern. In this response, we revise the manuscript to emphasize the necessity of mask freshness and quantify the potential attack surface when multiple purchases occur.}


\answer{We provide a formal analysis below to clarify the mask freshness.}
\answer{\input{revision/mask_freshness}}

\answer{\input{revision/assertion_signal}}
\answer{We revised Section~\ref{subsec:ot_selection} as follows:}

\revise{We require the masking matrices $({R}_P, {R}_N)$ to be refreshed for every verification session. Otherwise, colluding users could XOR masked instances obtained from different runs to cancel the masks and infer structural relationships between protected designs.}

\answer{We also enforce that the semantic map should expose a small subset of the design variables in Section~\ref{subsec:preprocess}.}

\revise{which correspond to a small subset of design variables. The semantic map assigns each observable signal a unique literal.}
    
\subsection{Requirements for Major Review}
\textbf{Q1:} Revise the threat model to address potential contradictions between "zero-trust" and "semi-honest" assumptions, specifically addressing resilience against malicious behaviors like aborts or bad inputs. What can each party learn? What fails in the malicious setting?


\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for pointing out the ambiguity. We have revised the threat model to clarify that “zero-trust” refers to eliminating trusted third parties rather than implying malicious security. We also specify what each party learns under the semi-honest assumption. The revised text in Section~\ref{sec:threat} is shown below.}

\revise{\input{revision/threatmodel}}

\textbf{Q2:} Provide a formal analysis of information leakage that addresses property probing via repeated queries, mask freshness, and potential security risks from user collusion. What are practical mitigations in case of leakage?


\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this important concern. In this response, we revise the manuscript to emphasize the necessity of mask freshness and quantify the potential attack surface when multiple purchases occur.}


\answer{We provide a formal analysis below to clarify the mask freshness.}
\answer{\input{revision/mask_freshness}}

\answer{\input{revision/assertion_signal}}
\answer{We revised Section~\ref{subsec:ot_selection} as follows:}

\revise{We require the masking matrices $({R}_P, {R}_N)$ to be refreshed for every verification session. Otherwise, colluding users could XOR masked instances obtained from different runs to cancel the masks and infer structural relationships between protected designs.}

\answer{We also enforce that the semantic map should expose a small subset of the design variables in Section~\ref{subsec:preprocess}.}

\revise{which correspond to a small subset of design variables. The semantic map assigns each observable signal a unique literal.}


\textbf{Q3:} Elaborate on limitations with respect to redistribution, as well as potential mitigation mechanisms to bind an IP to a certificate.


\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for the suggestion. Our framework focuses on
traceability rather than enforcing strict non-transferability. We revised the Section~\ref{subsec:ip-traceability} as the reviewer suggested as follows.}

\revise{\input{revision/redistribution}}

\textbf{Q4:} Expand the evaluation to include larger designs and comparative baselines (non-private SAT, ppSAT) to quantify the specific performance trade-offs of the privacy-preserving construction.


\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for this suggestion. In the following response, we first discuss the limitations of scaling \tool to large designs and then provide a quantitative comparison with non-private SAT.}

\answer{\input{revision/scalability}}

\answer{We acknowledge that privacy-preserving verification introduces a noticeable slowdown compared with the non-private baseline. Nevertheless, since verification is typically a one-time procedure before the IP transaction is finalized, the additional overhead remains acceptable in practice. We extend our evaluation in Section~\ref{subsec:nonprivate} as follows.}

\revise{\input{revision/non_ppsat}}

\textbf{Q5:} Discuss the practical challenges of integrating the framework with standard EDA toolchains and clarify the secure transmission of the control-flow-guided partial-order set to ensure it avoids information leakage.



\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this concern. In this response, we first discuss the integration of \tool into existing verification workflows, and then revise the manuscript to clarify the precise alignment required between the two parties. We clarify the transmission of the control-flow-guided partial-order set in Section~\ref{subsub:hwppsat}, which has been added to the manuscript. We then conduct extensive experiments to show that this optimization incurs negligible overhead in practice.}

\answer{\tool is designed to operate as a lightweight preprocessing and verification layer on top of existing verification flows rather than replacing them. In practice, hardware designs written in synthesizable RTL are first processed by any static-analysis frontend that can perform dataflow analysis. The design is then translated into an SMT representation and subsequently converted into CNF following the standard SAT-based hardware verification pipeline. \texttt{hw-ppSAT} serves as the checker that enables privacy-preserving formal verification. Although current commercial formal verification tools do not natively support such capabilities, the proposed framework can be integrated as an additional execution engine for existing verification tools such as VC Formal~\cite{synopsys:vcug} or JasperGold~\cite{JasperGold}.}

\answer{We also revised the Section~\ref{sec:con} to declare the alignment required between the two
parties. As shown below.}

\revise{A practical challenge of \tool lies in its interactive protocol, where stages such as oblivious design selection and secure SAT solving require synchronized message exchanges between the IP vendor and the IP user, introducing additional latency compared with offline verification. Despite this overhead, the framework remains compatible with existing post-licensing IP protection solutions and can be integrated into current hardware supply-chain ecosystems. Moreover, in realistic IP trading scenarios, verification is typically performed once prior to the transaction finalization.}


\answer{The control-flow-guided partial-order set is derived locally on the vendor side. Its transmission is protected by the OT protocol following the same mechanism described in Section~\ref{subsec:ot_selection}. We further provide the detailed revised script below.}

\answer{We further quantify the overhead of the OT-based heuristic retrieval in Figure~\ref{fig:heuristic_count}.
Among all benchmarks, \texttt{adbg} has the largest heuristic set, containing 308 literals. 
Even with a 128-bit encoding per literal, the total communication cost is approximately 4.8~KB, therefore the communication overhead introduced by retrieving $\heuset$ via OT is negligible compared to the design selection and verification phases in Section~\ref{subsec:overhead}.} 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/heuristic_literal_counts.pdf}
    \caption*{Fig.~\ref{fig:heuristic_count}: \answer{Number of literals in the control-flow-guided heuristic set ($\heuset$) for each benchmark design. Even for the largest design (\texttt{adbg}), the heuristic set contains only 308 literals, resulting in negligible communication overhead when retrieved via OT.}}
\end{figure}

\revise{Unlike \texttt{ppSAT.Solve}, \texttt{hw-ppSAT} requires the IP user to provide a partial-order set $\heuset$ as an additional input, which is generated on the IP vendor side.}

\revise{To prevent information leakage, the heuristic set associated with each IP design is retrieved through the same Oblivious Design Selection protocol described in Section~\ref{subsec:ot_selection}. Concretely, the IP vendor generates a heuristic set $\heuset^k$ for each design $\phi_k$ during preprocessing and includes it in the message vector used in the OT protocol. The IP user then retrieves the corresponding heuristic set using a 1-out-of-$N$ OT via
$$
(\heuset^i, \bot) \leftarrow {\sf OT}(i, \{\heuset^1, \heuset^2, \ldots, \heuset^N\}).
$$
By the security guarantee of OT, the user learns only $\heuset^i$ and obtains no information about $\{\heuset^j\}_{j\ne i}$, while the vendor learns nothing about the user's selection $i$. Furthermore, since $\heuset$ only specifies a partial ordering of variables for branching decisions, it does not reveal structural information about the underlying circuit.}


\textbf{Q6:} Discuss the robustness of hw-ppSAT on flattened netlists and quantify the efficiency gains of design pruning across various classes of properties and designs.

\noindent \textcolor{blue}{\textbf{Response:} We thank the reviewer for raising this important question.}

\answer{\input{revision/flatten_netlist}}

\answer{We revised the discussion in Section~\ref{subsec:preprocess} as follows.}

\revise{Existing translation tools built on hardware synthesis frameworks typically bind the design to a specific cell library and flatten it into gate-level netlists. 
Such flattening often removes high-level semantic structures, making it difficult to express verification properties that are naturally defined at the behavioral level. 
Moreover, complex operators (e.g., multiplexers) are decomposed into primitive logic gates, which introduces a large number of auxiliary variables and clauses during CNF generation. 
Since \tool encodes the CNF as a pair of binary matrices $(P, N) \in \{0,1\}^{n \times m}$, larger values of $n$ and $m$ directly increase the computational and communication overhead of the subsequent secure protocols.}


\answer{We have clarified the quantitative performance gains in Table~\ref{tab:exp}. Following the reviewer's suggestion, we have added a paragraph in Section~\ref{subsec:prune} to illustrate the impact of design pruning on various properties, as shown below.}

\revise{\input{revision/COI}}


\textbf{Q7:} Include quantitative data regarding the communication bandwidth overhead for the Oblivious Transfer and 2PC protocols.


\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for this suggestion. We extend our evaluation in Section~\ref{subsec:overhead} to quantify the communication overhead of both 2PC and OT. Overall, both OT and 2PC overhead scale approximately linearly with the design size, but design pruning and control-flow-guided heuristics significantly reduce the effective circuit size and number of giant steps, making privacy-preserving verification practical.}


\revise{
\input{revision/Crypto_overhead}}


\textbf{Q8:} Refine the related work comparison to clearly differentiate the proposed approach from methods in Table 1 (also correct ref [8] format).

\noindent \textcolor{blue}{\textbf{Response:}
We thank the reviewer for pointing this out. We have refined the related work to clearly differentiate \tool from existing methods, as shown below.}


\revise{\input{revision/related}}

\answer{In addition, the format of reference [8] has been corrected in the revised manuscript.}

\newpage






\begin{figure}[h]

    \centering
    \includegraphics[width=0.6\linewidth]{figs/assertion_used_over_design_pct.pdf}
    \caption{Percentage of design variables referenced by verification assertions relative to the total number of design variables across all benchmarks. The results show that verification properties typically involve only a small subset of the design variables (2.49\% on average).}
    \label{fig:assertion_signal}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/heuristic_literal_counts.pdf}
    \caption{Number of literals in the control-flow-guided heuristic set ($\heuset$) for each benchmark design. Even for the largest design (\texttt{adbg}), the heuristic set contains only 308 literals, resulting in negligible communication overhead when retrieved via OT.}
    \label{fig:heuristic_count}
\end{figure}

==> sections/secandpriv.tex <==
\section{Correctness and Efficiency}\label{sec:ceff}

\subsection{Correctness}

[sketch: correctness of transformation means correctness reduces to correctness of ppSAT]

\subsection{Efficiency Analysis}

[sketch: Using DLIS, complexity is $O(Smn + Sn \log n))$ where $S$ is the number of giant steps, which is nominally worst-case exponential, but in practice is often quite small, but also highly task specific so can only be analyzed empirically.]

\section{Security and Privacy}\label{sec:seca}

\subsection{Security Analysis}

[sketch: security reduces to ppSAT security, which reduces to boolean garbled circuit security. simulateability and composition of such functionalities is well-established, so all non-negligable information leakage is what the parties declare as inputs for the execution, and then the output + number of giant steps, note stronger security model than a TEE]

\subsection{Privacy Analysis}

[sketch: walk over each declared input from both parties, and justify that their exposure doesn't conflict with the goals of the BlindMarket system]
